Multiple-Relaxation Runge Kutta Methods for Conservative Dynamical Systems

We generalize the idea of relaxation time stepping methods in order to preserve multiple nonlinear conserved quantities of a dynamical system by projecting along directions defined by multiple time stepping algorithms. Similar to the directional projection method of Calvo et. al., we use embedded Runge-Kutta methods to facilitate this in a computationally efficient manner. Proof of the accuracy of the modified RK methods and the existence of valid relaxation parameters are given, under some restrictions. Among other examples, we apply this technique to Implicit-Explicit Runge-Kutta time integration for the Korteweg-de Vries equation and investigate the feasibility and effect of conserving multiple invariants for multi-soliton solutions.

==> img/article_file_2.tex <==
%===============================================================================
%===============================================================================
\renewcommand{\O}{{\mathcal O}}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}
\newcommand{\vardbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}

\newcommand{\Err}{\mathcal{I}(\zeta)}  
\newcommand{\myremarkend}{$\spadesuit$} 
\newcommand{\lbmap}{\left[} 
\newcommand{\rbmap}{\right]} 
\newcommand{\WSOset}{\mathbb{W}_q}
\newcommand{\OCset}{\mathbb{V}_{p}}
\newcommand{\numc}{n_c}
\newcommand{\minPolc}{P_{\rm C}}
\newcommand{\qso}{\tilde{q}}
\newcommand{\RzCoeff}{\beta}
\newcommand{\Sredr}{\tilde{r}}
\newcommand{\BigO}{{\mathcal{O}}}
\newcommand{\Dt}{\Delta t}
\newcommand{\vecpower}[2]{\vec{#1}^{\,#2}}
\newcommand{\kgen}{m}
\newcommand{\basismat}{L}
\newcommand{\Umat}{U}
\newcommand{\Vmat}{V}
\newcommand{\Wmat}{W}
\newcommand{\bsmall}{\hat{\vec{b}}}
\newcommand{\Ksmall}{\hatK}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\bk}{\vec{b}^{\,k}}
%=========================
\newcommand{\kibitz}[2]{\textcolor{#1}{#2}}
\newcommand{\abhi}[1] {\kibitz{red}{[AB says: #1]}}
%=========================


	\section{Introduction}
    The development of structure-preserving time integrators, which preserve qualitative properties of initial value problems, has been a major focus of numerical analysis for the last few decades. Here we are interested in conserved quantities preserved by the true solution of a system of differential equations.  Consider an autonomous ordinary differential equation initial-value problem
    \begin{equation}\label{IVP_1}
             \dot{u}(t)  = f\left(t,u(t)\right), \  u(0) = u_{0}, \ u(t)\in \Real^{m} \;,
    \end{equation}
    where $ \ f : \mathcal{D} \subset \Real^m \to \Real^m$ is a sufficiently smooth function. We say that the problem \eqref{IVP_1} has $\ell$ conserved quantities defined in terms of a $\mathcal{C}^{1}(\mathcal{\bar{D}})$ function $ \ G: \mathcal{\bar{D}} \subset \Real^{m} \to \Real^{\ell}$ if
    % if the solution $u(t)$ of \eqref{IVP_1} belongs to  $\mathcal{M} := \left\{u\in \Real^m: G(u) = G(u_{0}) \right\}$ and 
    \begin{align*}
        \frac{\textrm{d}}{\textrm{dt}}G(u(t)) = \nabla G(u(t))^{T}f(t,u(t)) = 0 \;.
    \end{align*}
    %This $\ell$-invariant function $G$ is also called weak invariant \cite{haier2006geometric} of \eqref{IVP_1} and it depends on initial conditions. A sufficiently smooth scalar function $ \ I: \mathcal{D} \subset \Real^{m} \to \Real$ is called a strong invariant or a first integral if 
    %\begin{align*}
    %    \nabla I(u)^{T}f(u) = 0, \ u \in \mathcal{D}\;.
    %\end{align*}
    %Strong invariants do not depend on the initial conditions and $I(u(t))$ is constant for all solutions $u(t)$ of the differential system. 
    Time-dependent differential equations with multiple conserved quantities (mass, energy, etc.) appear in many applications. Examples include special classes of ordinary differential equations (for example, the Lotka-Volterra system), Hamiltonian systems,
    %(the classic example is Kepler's two-body problem), 
    and many partial differential equations, including the Korteweg-de Vries (KdV) equation, nonlinear Schrodinger equation, etc. Since in general numerical integrators do not conserve invariants of the systems, in recent years the preservation of invariants has grown in significance as a criterion of a numerical scheme's effectiveness \cite{li1995finite}. Failure to maintain the invariants sometimes leads to non-physical numerical solutions \cite{gear1992invariants} or spurious blow-up of the numerical solutions \cite{arakawa1997computational} when numerically integrating the system. In many cases, conservative schemes are also proved to have better error growth behavior over time than nonconservative methods \cite{de1997accuracy,duran2000numerical}. In such cases, conservative methods may be the only approach that gives acceptable numerical solutions for long-time simulations.  Further studies illustrating the superiority of conservative approaches over generic methods in this regard can be found in \cite{calvo1993development, cano1997error,calvo2011error,ranocha2021rate}.
    
    Runge-Kutta methods are among the most widely used time-integration techniques, and it is natural to consider these methods while studying invariant preserving numerical integrators. All Runge-Kutta methods preserve linear invariants.  Only symplectic RK methods preserve quadratic invariants \cite{cooper1987stability}, and such methods must be fully implicit.  It is also well-known \cite{haier2006geometric} that no Runge-Kutta method can preserve all polynomial invariants of degree $n \geq 3$. This restriction motivates the development of new techniques that can preserve general conserved quantities.
    
    Multiple approaches have been introduced to overcome the shortcomings mentioned above in the existing numerical integrators, including for example, discrete gradients and orthogonal projection.  Here we review the ideas leading to relaxation methods. 
 Dekker and Verwer introduced a modification of the classical 4th-order explicit RK method in order to preserve a quadratic invariant \cite{dekker1984stability}.  This modification can be viewed as projection onto the conservative manifold along an oblique direction.  Similar ideas were further developed and generalized by Calvo and coauthors to allow the use of other explicit RK methods and the preservation of multiple, not necessarily quadratic, invariants \cite{calvo2006preservation}, at the cost of a reduction by one in the order of convergence of the method.
 A major advantage of these oblique projection techniques when compared with orthogonal projection is that oblique projection can be designed to maintain preservation of linear invariants (which are naturally preserved by RK methods) while also preserving nonlinear invariants.
Recently, a further modification of these ideas, known as  relaxation \cite{ketcheson2019relaxation,ranocha2020relaxation_1} has been proposed in order to impose dissipation or conservation of general nonlinear functionals while retaining the full accuracy of the original method. This approach was successfully applied to Hamiltonian systems \cite{ranocha2020relaxation} and was further generalized in the context of multistep methods \cite{ranocha2020general}. 
    
    So far, relaxation methods have been used to conserve a single invariant of a system. Preserving a single generic invariant requires solving a nonlinear equation for one relaxation parameter at each time step of the method. In this work we generalize the idea of relaxation in order to preserve multiple invariants, similar to what was done for the incremental direction technique in \cite{calvo2006preservation}.  In order to preserve multiple invariants we require multiple linearly-independent search directions, which could be obtained in principle from any set of distinct time discretizations.  Following the natural and efficient approach used in \cite{calvo2006preservation}, we employ sets of embedded RK methods so that no additional RHS evaluations are needed.
    Compared to the incremental direction technique \cite{calvo2006preservation}, the relaxation approach requires one fewer embedded methods and converges at a rate one order higher.  
    %Conserving $\ell(\geq 1)$ invariants by the relaxation approach needs to solve a nonlinear system for $\ell$ relaxation parameters at each time step. 
    We provide a more detailed investigation of the feasibility and effectiveness of solving the required algebraic equations, as well as showing applications to a PDE with mutliple conserved quantities.
    
    The main contributions of this work are: (a) the generalization of the relaxation approach to conserving several invariants, (b) proof of the existence of relaxation parameters, and (c) the demonstration of the benefits of preserving more than one invariant via several numerical examples. 
    %In section 2, we briefly review relaxation RK methods for one invariant and generalize this approach for several invariants in section 3. The proof of the existence of relaxation parameters is given in section 4. Several numerical experiments are carried out in section 5 to demonstrate how our methodology performs on several test problems. Finally, we close with a conclusion in section 6.
    
	\section{Runge-Kutta Methods and Their Relaxation Versions}
	An $\mathrm{s}$-stage RK method can be represented via its \emph{Butcher tableau}:
    \begin{equation}\label{B_table_RK}
        \renewcommand\arraystretch{1.2}
        \begin{array}
            {c|c}
            \vec{c} & A\\
            \hline
            & \vec{b}^{\,T}
        \end{array}\;, 
    \end{equation}
    where the matrix $A = (a_{ij})\in \Real^{s \times s}$ and vector $\vec{b} \in \Real^{s}$.  We assume 
    \begin{align} \label{c-assumption}
    \vec{c} = A\vec{e},
    \end{align}
    where $\vec{e}$ is the vector of ones in $\Real^{s}$.
    
	For an initial value problem
    \begin{equation}\label{IVP_2}
             \dot{u}(t)  = f\left(t,u(t)\right), \  u(0) = u_{0}; \ u\in \Real^{m}, \ f : \Real\times\Real^m \to \Real^m,
    \end{equation}
    method \eqref{B_table_RK} provides the numerical solution
    \begin{subequations}\label{RK_methods}
        \begin{align}
            g_i & = u^n+\Delta t \sum_{j = 1}^{s} a_{ij} f(t_n+c_j \Delta t, g_j), \ i = 1,2, \ldots,s \;, \label{RK_methods_a}\\
            u(t_n+\Dt) \approx u^{n+1} & = u^{n}+\Delta t \sum_{j = 1}^{s} b_j f(t_n+c_j \Delta t, g_j)\;, \label{RK_methods_b}
        \end{align}
    where $\Delta t$ is a time step size, $u^n$ and $u^{n+1}$ are the numerical approximations to the true solution at time $t_n$ and $t_{n+1} = t_n+\Delta t$, respectively. Assume that the system \eqref{IVP_2} has a scalar conserved quantity $G_1:\Real^{m} \to \Real$, i.e., $G_1$ remains constant along each solution. In general, RK methods do not preserve this qualitative behavior discretely. To remedy this one may use a slight modification (known as relaxation) \cite{ketcheson2019relaxation,ranocha2020relaxation_1,ranocha2020relaxation} in which the update
    \begin{align}\label{RRK_methods_1}
        u(t_n+\gamma\Dt) \approx u^{n+1}_{\gamma} & = u^{n}+\gamma \Delta t \sum_{j = 1}^{s} b_j f(t_n+c_j \Delta t, g_j),
    \end{align}
    \end{subequations}
    is used instead of \eqref{RK_methods_b}, where $\gamma \in \Real$ is a scalar that is chosen by imposing the discrete conservation property 
    \begin{align} \label{eq:conservation}
       G_1(u^{n+1}_{\gamma})  =  G_1(u^{n}) \;.
    \end{align}
    The nonlinear algebraic equation \eqref{eq:conservation} must be solved at each time step.  For a $p$th-order baseline RK method, it can be shown that there exists a solution satisfying $\gamma = 1+\mathcal{O}(\Delta t^{p-1})$ (under some restrictions) \cite{ketcheson2019relaxation,ranocha2020relaxation_1}. Consequently, the relaxation RK method defined by \eqref{RK_methods_a} and \eqref{RRK_methods_1} has order $p$ when the new updated solution is interpreted as an approximation of the true solution at time $t_n+\gamma \Delta t$. 

\subsection{Embedded Runge-Kutta Sets}

    In the next section we extend the relaxation idea to enforce conservation of multiple invariants.  In order to do so, we require multiple candidate new solutions $u^{n+1}$ that are all of sufficient accuracy.  A convenient and inexpensive way to obtain such solutions utilizes the concept of embedded RK methods.  

    We say a set of RK methods is embedded if all methods in the set share the same coefficient matrix $A$, with different weight vectors $b$.
    Thus the $k$th method in the set has coefficients
    denoted by $(A,\vec{b}^{\,k})$.  
    The accuracy of a solution involving all methods in the set will be governed by the order of the least accurate method, so we define
    \begin{align}
    p_{\min} = \min_k p_k
    \end{align}
where $p_k$ is the order of method $(A,\bk)$.
    To apply such a set of methods, the stage equations \eqref{RK_methods_a}
    need only be solved once, after which the simple arithmetic updates
     \begin{align}\label{RK_methods_1}
        u^{n+1,k} & = u^{n}+\Delta t \sum_{j = 1}^{s} b_j^k f(t_n+c_j \Delta t, g_j),
    \end{align} 
    can be computed.  No additional evaluations of $f$ or solutions of algebraic equations are required.
    
    Traditional use of embedded methods has focused on pairs, in which one method is designed to have lower order and the difference between the two solutions is used as an estimate of the local error.  Here, in contrast, we will make use of sets consisting of $\ell\ge 2$ methods, and solutions from all methods in the set will be used as part of the numerical solution update.  Ideally, all methods in the set would have the same order of accuracy.  In the numerical examples in this work, we mainly make use of existing methods (for which the method orders differ), and leave the design of RK sets with equal order of accuracy to future work.
    
	\section{Generalization of Relaxation Runge-Kutta Methods for Multiple Invariants}
	So far the relaxation approach has been applied to conserve one quantity of a differential system. We generalize this methodology to conserve multiple nonlinear invariants. We assume that the system of differential equations has $\ell$ smooth invariant  functions $G_1(u)$, $G_2(u)$,...,$G_{\ell}(u)$ defined in a solution space in $\mathbb{R}^m$ and define
    \begin{align} \label{l-invariants}
        G := (G_1,G_2, \ldots, G_{\ell})^{T}: \mathbb{R}^m \to \mathbb{R}^{{\ell}} \;.
    \end{align}
    The basic idea to conserve $\ell \geq 1$ invariants is to use a set of ${\ell}$ linearly-independent embedded RK methods (each of order at least 2) and find a suitable direction in the plane spanned by directions induced by those ${\ell}$ methods so that the invariants are preserved:
    \begin{align} \label{relaxation-equations}
        G(u^{n+1}_{\vec{\gamma}}) & = G(u^n).
    \end{align}
    Here the updated solution $u^{n+1}_{\vec{\gamma}}$ is computed using given ${\ell}$ linearly-independent embedded RK methods as
    \begin{subequations}\label{modified_Update_rule}
        \begin{align}
            u^{n+1}_{\vec{\gamma}}  & := u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \;, \label{modified_Update_rule_a} \\
            d_{k}^{n} & :=\sum_{j = 1}^{s} b_{j}^{k} f(t_n+c_j \Delta t, g_j), \ \text{for} \ k = 1,2,...,{\ell}\;, \label{increments}
        \end{align}
    \end{subequations}
    where $u^{n+1}=u^{n}+ \Delta t d_{1}^{n}$, $\vec{\gamma} = (\gamma_{1},\gamma_{2},\ldots, \gamma_{{\ell}}) \in \Real^{\ell}$, and stage values $g_i$'s are defined in \eqref{RK_methods_a}. The directions are computed according to given embedded RK methods $(A,\vec{b}^1,\vec{b}^2,\cdots,\vec{b}^{\ell})$
	where, by convention, the first method defined by the vector ${\vec{b}^1} = [b^{1}_{1},b^{1}_{2},\ldots, b^{1}_{s}]^T$ is used to compute $u^{n+1}$. At each step, we now require to solve a nonlinear system of $\ell$ equations in $\ell$ unknowns $(\gamma_1, \gamma_2,…,\gamma_{\ell})$.In the case  $\ell = 1$, this reduces to the usual relaxation approach. We refer to these generalized methods as multiple relaxation Runge-Kutta methods.

	\section{Existence of Relaxation Parameters and Accuracy of the Methods}
   \begin{lemma}
        Suppose that the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants}, and let a set of embedded Runge-Kutta methods $(A,\vec{b}^{\,1},\dots,\vec{b}^{\,\ell})$, with $p_{\min}:=p\geq 2$ be given. Let $u^n = u(t_n) \in \Real^m$, $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$  with $d_{k}^{n}$ defined in \eqref{increments}, computed with a time step  $\Delta t \ge 0$, and $u^{n+1} = u^n+\Delta t d_{1}^{n}$. If 
        \begin{align}\label{grad_assumption}
            \nabla G(u^{n+1}) \cdot D_n = B(u^n)\Delta t+\O(\Delta t^2)
        \end{align}     
        holds with non-singular $B(u^n)$ and $||B^{-1}||=\O(1)$, then there exists $\Delta t^{*} > 0$ such that for every $\Delta t \in [0,\Delta t^{*}]$ there is a unique vector $\vec{\gamma}$ 
        such that equations \eqref{relaxation-equations}-\eqref{modified_Update_rule} are satisfied and 
        $$\gamma_{i} = \O(\Delta t^{p-1}), \ \text{for } \ i = 1,2,\cdots, \ell.$$
    \end{lemma}
    \begin{proof}
        Consider the real function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
        \begin{align}\label{Lemma_eq1}
            g(\tau, \vec{\gamma}) :=      
           \frac{G\left(u^{n+1}+\tau \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}\right)- G(u^{n})}{\tau^2}, & \ \text{for} \ \tau \neq 0 \;.
        \end{align}
        % Applying Taylor's theorem with $h_n  := \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}$ we obtain 
        % \begin{align}\label{Lemma1_eq2}
        %      G\left(u^{n+1}+ \tau h_n\right) = G(u^{n+1}) + \tau \nabla G(u^{n+1}) \cdot h_{n} + \tau^2 \frac{D^2g(u^{n+1})}{2!}(h_{n},h_{n}) +\O(\tau^3).
        % \end{align}
        Note that the numerical solution of an RK method of order $p_{\min} = p$ satisfies (with the assumption $u^{n} = u(t_n)$)
        \begin{align*}
            G_i(u^{n+1})- G_i(u^{n}) & = G_i\left(u(t_{n+1})+\O(\Delta t^{p+1})\right) - G_i\left(u(t_{n})\right) \\
            & = G_i\left(u(t_{n+1})\right) - G_i\left(u(t_{n})\right) +\O(\Delta t^{p+1}) \\
            & = \O(\Delta t^{p+1})\;. 
        \end{align*}
        This holds for $i=1,2,\cdots, \ell$ and hence 
        \begin{align}\label{accuracy_diff_G}
            G(u^{n+1})- G(u^{n}) = \O(\Delta t^{p+1}) \;.
        \end{align}
        Using Taylor's theorem with $h_n  := \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}$, the assumption \eqref{grad_assumption}, and equation \eqref{accuracy_diff_G} in \eqref{Lemma_eq1} we write
        \begin{align*}\label{Lemma1_eq3}
             g(\Delta t, \vec{\gamma}) & = \Delta t^{-2} \left[ G\left(u^{n+1}+ \Delta t h_n\right) - G(u^{n})\right]  \\
             & = \Delta t^{-2} \left[ G(u^{n+1}) + \Delta t \nabla G(u^{n+1}) \cdot h_{n} + \Delta t^2 \frac{D^2g(u^{n+1})}{2!}(h_{n},h_{n}) +\O(\Delta t^3) - G(u^{n})\right]  \\
             & = \frac{G(u^{n+1})- G(u^{n})}{\Delta t^2} + \Delta t^{-1} \nabla G(u^{n+1}) \cdot D_{n} \vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n}) +\O(\Delta t)  \\
             & = \O(\Delta t^{p-1}) + \left(B(u^n)+\O(\Delta t)\right)\vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})+\O(\Delta t)\\
             & = \left(B(u^n)+\O(\Delta t)\right)\vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})+\O(\Delta t) \ \text{since} \ p \geq 2 \;.
        \end{align*}
        Thus we define, 
        \begin{align}
            g(0,\vec{\gamma}):=\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = B(u^n)\vec{\gamma}+\left. \frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})\right|_{\Delta t = 0}\;,
        \end{align}
        and then $g(\Delta t,\vec{\gamma})$ is continuous for all $\Delta t \geq 0$. Notice that $g(0,\vec{0}) = 0$. Furthermore, the function is differentiable with respect to $\Vec{\gamma}$ and the Jacobian is given by
        $$J_{g,\vec{\gamma}}(0,\vec{0}) = B(u^n).$$
        Since $B(u^n)$ is non-singular by assumption, the implicit function theorem guarantees the existence of a $\Delta t^{*} > 0$ and a unique function $$\vec{\gamma}(\Delta t) = \left(\gamma_1(\Delta t), \gamma_2(\Delta t),\ldots, \gamma_{\ell}(\Delta t)\right)$$
        such that, for any $\Delta t \in [0,\Delta t^{*}]$ we have $\vec{\gamma}(0) = \vec{0}$ and $g(\Delta t,\vec{\gamma}(\Delta t)) = 0$. Hence it follows from \eqref{Lemma_eq1} that the method defined in \eqref{modified_Update_rule} applied with this set of relaxation parameters will satisfy the $\ell$-invariant equations given by \eqref{relaxation-equations} for the system. 
        
        To know the accuracy of $\vec{\gamma}$ consider the expansion
        \begin{align}\label{Lemma1_eq4}
            g(\Delta t,\vec{\gamma}) = g(\Delta t,\vec{0}) + J_{g,\vec{\gamma}}(\Delta t,\vec{0}) \cdot \vec{\gamma} + \mathcal{O}(||\vec{\gamma}||^2) 
        \end{align}
        with 
        \begin{align}\label{Lemma1_eq5}
            g(\Delta t,\vec{0}) = \frac{G(u^{n+1})- G(u^{n})}{\Delta t^2} = \mathcal{O}(\Delta t^{p-1}), \ \text{by} \ \eqref{accuracy_diff_G} \;,
        \end{align} 
        and 
        \begin{align}\label{Lemma1_eq6}
            J_{g,\vec{\gamma}}(\Delta t,\vec{0}) = J_{g,\vec{\gamma}}(0,\vec{0}) + \mathcal{O}(\Delta t) = B(u^n) +\mathcal{O}(\Delta t) \;. 
        \end{align}
        Using \eqref{Lemma1_eq4}, \eqref{Lemma1_eq5}, \eqref{Lemma1_eq6}, and the assumption $||B^{-1}||=\O(1)$ we conclude that each component of the vector $\vec{\gamma}$ is $\mathcal{O}(\Delta t^{p-1})$.     
    \end{proof}

    \begin{theorem}
        Suppose the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants} and let $(A,\vec{b}^{\,1},\dots,\vec{b}^{\,\ell})$ be the coefficients of a set of $\ell$ embedded Runge-Kutta methods with $p_{\min}:=p\geq 2$. Consider the generealized relaxation method defined by \eqref{relaxation-equations}-\eqref{modified_Update_rule} and assume $\vec{\gamma} = \O(\Delta t^{p-1})$. Then:
        \begin{enumerate}
            \item If the solution $u^{n+1}_{\vec{\gamma}}$ is interpreted as an approximation to $u(t_n+\Delta t)$, the method has order $p-1$.
            \item The generalized relaxation method interpreting $u^{n+1}_{\vec{\gamma}}$ as an approximation to $u(t^{n+1}_{\vec{\gamma}})$ has order $p$, where $t^{n+1}_{\vec{\gamma}}=t_n+\left(1+\sum \gamma_{i} \right)\Delta t$.
        \end{enumerate}
    \end{theorem}
    \begin{proof}
        Let $\mathbf{f} := [f(t_n+c_1 \Delta t, g_1)|f(t_n+c_2 \Delta t, g_2)| \ldots| f(t_n+c_s \Delta t, g_s)]$ be the matrix of stage vectors, $\mu_1 := 1+\gamma_1$, and $\mu_i := \gamma_i$ for $i = 2,3,\cdots, \ell$. Then the modified update rule \eqref{modified_Update_rule_a} can be rewritten as
        \begin{equation}
            \begin{aligned}
                u^{n+1}_{\vec{\gamma}} & = u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}  \\
                & = u^{n}+\Delta  t \sum_{i=1}^{{\ell}} \mu_{i} \mathbf{f} \vec{b}^{i} \ \text{using} \ \eqref{increments} \\
                & = u^{n}+\Delta  t \mathbf{f}  \sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\;. \\
            \end{aligned}
        \end{equation}
        So we can view the update rule of the generalized relaxation method as applying the following RK method to the system:
        \begin{equation}\label{diff_formulation_GRRRK_mthd}
            \renewcommand\arraystretch{1.2}
            \begin{array}
            {c|c}
            \vec{c} & A\\
            \hline
            & \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{\,T}
            \end{array}\;.
        \end{equation}
        Following the proof of \cite[Theorem 2.7]{ketcheson2019relaxation}, we use an equivalent set of order conditions \cite{albrecht1996runge}
        \begin{subequations}
            \begin{align}
                \vec{b}^{\,T}\vec{c}^{\, k-1} - 1/k & = 0, & 1 \le k \le p, \\
                \vec{b}^{\,T} v & = 0 & \forall v \in V_{p},
            \end{align}
        \end{subequations}
        for an RK method \eqref{B_table_RK} to have order $p$, where $V_{p}$ is a set of vectors depending only on $A$. 
        
        If $u^{n+1}_{\vec{\gamma}} \approx u(t_n+\Delta t)$, in view of \eqref{diff_formulation_GRRRK_mthd}, the order conditions for the generalized relaxation RK methods can be obtained by replacing $\vec{b}^{\,T}$ with $\left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}$:
        \begin{subequations}
            \begin{align}
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - 1/k & = 0, & 1 \le k \le p, \label{IDT_OC_a} \\
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T} v & = 0 & \forall v \in V_{p}, \label{IDT_OC_b}
            \end{align}
        \end{subequations}
        Since each of the embedded methods has order $p$, it follows that for all $i$, $(\vec{b}^{i})^{\,T} v = 0, \ \forall \ v \in V_{p}$ and hence \eqref{IDT_OC_b} is satisfied. On the other hand, the accuracy of $\mu_i$'s and the order of embedded methods implies that the left-hand side of equation \eqref{IDT_OC_a} is $\O(\Delta t^{p-1})$. This quantity gets multiplied by $\O(\Delta t^{k})$ in the error expansion producing the leading order term $\O(\Delta t^{p})$; hence the method has order $p-1$.
        
        When we interpret the solution $u^{n+1}_{\vec{\gamma}}$ as an approximation to $u(t^{n+1}_{\vec{\gamma}}) = u(t_n+\left(\sum \mu_{i} \right)\Delta t)$, we view the numerical solution $u^{n+1}_{\vec{\gamma}}$ as an interpolant of the RK method's \eqref{diff_formulation_GRRRK_mthd} solution, evaluated at $\left(\sum \mu_{i} \right)\Delta t$. Then the set of order conditions for this interpolated solution becomes
        \begin{subequations}
            \begin{align}
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - \frac{\left(\sum \mu_{i} \right)^k}{k} & = 0, & 1 \le k \le p, \label{GRRRK_OC_a} \\
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T} v & = 0 & \forall v \in V_{p}. \label{GRRRK_OC_b}
            \end{align}
        \end{subequations}
        Notice that equation \eqref{GRRRK_OC_b} is the same as condition \eqref{IDT_OC_b}, so the order conditions in \eqref{GRRRK_OC_b} are satisfied. It is easy to see that the equation in \eqref{GRRRK_OC_a} for $k=1$ is also exactly satisfied. For $k \geq 2$, we write 
        \begin{align*}
            \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - \frac{\left(\sum \mu_{i} \right)^k}{k} & =  \sum_{i=1}^{{\ell}} \frac{\mu_{i}}{k}  - \frac{\left(\sum \mu_{i} \right)^k}{k}  \\
            & = \frac{\sum \mu_{i}}{k} \left(1-\left(\sum \mu_{i}\right)^{k-1}\right)\\
            & = \frac{\sum \mu_{i}}{k} \left(1-\left(1+\O(\Delta t^{(p-1)(k-1)})\right)\right) \\
            & = \O\left(\Delta t^{(p-1)(k-1)}\right) \;.
        \end{align*}
        Each of these residuals gets multiplied by $\O(\Delta t^k)$ in the error expansion, and the error term becomes $\O\left(\Delta t^{(k-1)p+1}\right)$. This makes the leading order error term $\O\left(\Delta t^{p+1}\right)$ for $k \ge 2$; hence, the method has order $p$.
    \end{proof}
    
    % \begin{theorem}
    %     Let $u^n \in \Real^m$, a set of embedded Runge-Kutta methods $(A,b^1,\dots,b^\ell)$, and $\Delta t \ge 0$ be given.  Let $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$  with $d_{k}^{n}$ defined in \eqref{increments}.
    %    Suppose that the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants}
    %    %defined by the map $G: \mathbb{R}^m \to \mathbb{R}^{\ell}$, $G(u) := (G_1(u),G_2(u), \ldots, G_{\ell}(u))^{T}$, 
    %    and that 
    %    $$\left(\nabla G(u^{n})\right)^{T} \cdot D_n = M(u^n)$$
    %     holds with non-singular $M(u^n)$.  Then there exists $\Delta t^{*} > 0$ such that for every $\Delta t \in [0,\Delta t^{*}]$ there is
    %      a unique vector $\vec{\gamma}$ %$\left(\gamma_1(u^n,\Delta t), \gamma_2(u^n,\Delta t),\ldots, \gamma_{\ell}(u^n,\Delta t)\right)$ 
    %     such that equations \eqref{relaxation-equations}-\eqref{increments} are satisfied.

    %     Let $p$ denote the minimum order of accuracy of the Runge-Kutta methods in the set.  Then
    %     $$
    %         u^{n+1}_{\vec{\gamma}} = u\left(t_n+\left(1+\sum_i \gamma_i\right) \Delta t\right) + {\mathcal O}(\Delta t^{p+1}).
    %         $$
    % \end{theorem}
    % \begin{proof}
    %     % Consider the function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
    %     % \begin{align}\label{Existence_proof_eq1}
    %     %     g(\Delta t, \vec{\gamma}) :=
    %     %     \begin{cases}
    %     %                  \frac{G\left(u^{n+1}_{\vec{\gamma}}\right)- G(u^{n})}{\Delta t} & \text{if} \ \Delta t \neq 0 \\
    %     %                  C^{*} &  \text{if} \ \Delta t = 0 \;,
    %     %     \end{cases}
    %     % \end{align}
    %     % where $C^{*}$ is defined as $C^{*} := \displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = \nabla G(u^{n}) \cdot \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right)$.
        
    %     % {\color{blue} With $h_n  := \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right) $, we write
    %     % \begin{align*}
    %     %     g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^n+ \Delta t h_n\right) - G(u^{n})\right] \\
    %     %     & = \frac{1}{\Delta t} \left[ G(u^n) + \Delta t \nabla G(u^n) \cdot  h_n + \mathcal{O}(\Delta t^2)  - G(u^{n})\right].
    %     % \end{align*}
    %     % Hence $\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} =\nabla G(u^n) \cdot  h_n = \nabla G(u^{n}) \cdot \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right)$.
    %     % }
        
    %     % Since $G$ is a continuously differentiable function, using the mean value theorem we obtain 
    %     % \begin{align*}
    %     %      G\left(u^n+ \Delta t h_n\right) - G(u^{n}) = \left(\int_{0}^{1} \nabla G(u^n + \theta \Delta t h_n ) \ d\theta \right) \cdot \Delta t h_n.
    %     % \end{align*}
    %     % Then for $\Delta t \neq 0$ we have 
    %     % \begin{align}\label{Existence_proof_eq2}
    %     %      g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^n+ \Delta t h_n\right) - G(u^{n})\right] = \left(\int_{0}^{1} \nabla G(u^n + \theta \Delta t  h_n ) \ d\theta \right) \cdot h_n.
    %     % \end{align}
        
    %     Consider the function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
    %     \begin{align}\label{Existence_proof_eq1}
    %         g(\Delta t, \vec{\gamma}) :=      
    %              \frac{G\left(u^{n+1}_{\vec{\gamma}}\right)- G(u^{n})}{\Delta t}, & \ \text{for} \ \Delta t \neq 0 \;,    
    %     \end{align}
        
    %     where $g(0,\vec{\gamma})$ is given by the corresponding limit 
    %     \begin{align}
    %         g(0, \vec{\gamma}):=\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} =\nabla G(u^{n+1}) \cdot  h_n + \mathcal{O}(\Delta t)= \nabla G(u^{n}) \cdot h_n  \;,
    %     \end{align}
    %     where $h_n  := \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}$.
    %     Since $G$ is a continuously differentiable function, using the mean value theorem we obtain 
    %     \begin{align*}
    %          G\left(u^{n+1}+ \Delta t h_n\right) = G(u^{n+1}) + \left(\int_{0}^{1} \nabla G(u^{n+1} + \theta \Delta t h_n ) \ d\theta \right) \cdot \Delta t h_n.
    %     \end{align*}
    %     Then for $\Delta t \neq 0$ we have 
    %     \begin{align}\label{Existence_proof_eq2}
    %          g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^{n+1}+ \Delta t h_n\right) - G(u^{n})\right] \\
    %          & = \frac{G(u^{n+1})- G(u^{n})}{\Delta t}+\left(\int_{0}^{1} \nabla G(u^{n+1} + \theta \Delta t  h_n ) \ d\theta \right) \cdot h_n.
    %     \end{align}
        
        
    %     Using \eqref{Existence_proof_eq2}, we conclude that $\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = \nabla G(u^{n}) \cdot h_n$, and hence $g$ is continuous function at $\Delta t = 0$. Taking into account the smoothness of $G$, it is easy to see that $g$ is differentiable with respect to $\vec{\gamma}$ and the derivative is also a continuous in a neighbourhood of the origin. Observe that $g(0,\vec{0}) = \vec{0}$ and the Jacobian is given by
    %     \begin{align}
    %         J_{g,\vec{\gamma}}(0,\vec{0}) = (\nabla G(u^n))^T \cdot D_n = M(u^n) \;,
    %     \end{align}
    %     where $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$. 
    %     {\color{blue}
    %     \begin{align*}
    %            J_{g,\vec{\gamma}}(\Delta t,\vec{\gamma}) = & \frac{1}{\Delta t}
    %             \begin{bmatrix}
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n}\\
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n}\\
    %                 \vdots & \\
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n} \;,
    %             \end{bmatrix} \\
    %             & = (\nabla G(u^{n+1}_{\vec{\gamma}}))^T \cdot D_n \;.
    %     \end{align*}
    %     }
    %     Since $M(u^n)$ is non-singular by assumption, the implicit function theorem guarantees the existence of a $\Delta t^{*} > 0$ and a unique set $$\left(\gamma_1(u^n,\Delta t), \gamma_2(u^n,\Delta t),\ldots, \gamma_{\ell}(u^n,\Delta t)\right)$$
    %     such that, for any $\Delta t \in [0,\Delta t^{*}]$ we have $g(\Delta t,\vec{\gamma}) = 0$. Hence the method defined above applied with these set of relaxation parameters, will preserve $\ell$ invariants for the system. 
        
    %     Consider the expansion
    %     \begin{align}\label{Existence_proof_eq3}
    %         g(\Delta t,\vec{\gamma}) = g(\Delta t,\vec{0}) + J_{g,\vec{\gamma}}(\Delta t,\vec{0}) \cdot \vec{\gamma} + \mathcal{O}(||\vec{\gamma}||^2) 
    %     \end{align}
    %     with \begin{align}\label{Existence_proof_eq4}
    %         g(\Delta t,\vec{0}) = \frac{G(u^{n+1})- G(u^{n})}{\Delta t} = \mathcal{O}(\Delta t^p) \;,
    %     \end{align} 
    %     and 
    %     \begin{align}\label{Existence_proof_eq5}
    %         J_{g,\vec{\gamma}}(\Delta t,\vec{0}) = J_{g,\vec{\gamma}}(0,\vec{0}) + \mathcal{O}(\Delta t) = M(u^n) +\mathcal{O}(\Delta t) \;. 
    %     \end{align}
    %     Using \eqref{Existence_proof_eq3}, \eqref{Existence_proof_eq4}, and \eqref{Existence_proof_eq5} we conclude that each component of the vector $\vec{\gamma}$ is $\mathcal{O}(\Delta t^p)$.
    %     The accuracy of the $p$th order baseline method and each $\gamma_{i}$ being $\mathcal{O}(\Delta t^p)$ imply that 
    %     \begin{equation}\label{Existence_proof_eq6}
    %         \begin{aligned}
    %         u^{n+1}_{\vec{\gamma}} & = u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \\
    %         & = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1})\;.
    %         \end{aligned}
    %     \end{equation}

    %     On the other hand when the numerical solution is considered as an approximation at $t^{n+1}_{\vec{\gamma}} = t^{n+1}+\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}$, using Taylor expansion we obtain 
    %     \begin{align}\label{Existence_proof_eq7}
    %         u(t^{n+1}_{\vec{\gamma}}) = u(t_{n+1}) + \dot{u}(t_{n+1})\left(\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}\right) + \mathcal{O}\left(\left(\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}\right)^2\right) = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1}) \;.
    %     \end{align}
    %     The result $u^{n+1}_{\vec{\gamma}} - u(t^{n+1}_{\vec{\gamma}}) = \mathcal{O}(\Delta t^{p+1}) $ follows from \eqref{Existence_proof_eq6} and \eqref{Existence_proof_eq7}, and hence the relaxation method has order $p$.

        
    %     % The accuracy of the $p$th order baseline method and the $(p-1)$th order embebdded method imply that 
    %     % \begin{align}
    %     %     u^{n+1} = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1}) \ \text{and} \  u^{n+1,i} = u(t_{n+1}) + \mathcal{O}(\Delta t^{p}) \;,
    %     % \end{align}
    %     % where $u^{n+1}=u^{n}+\Delta t d_{1}^{n}$ and $u^{n+1,i} = u^{n}+\Delta t d_{i}^{n}$ are the approximate solutions by the baseline method and the $i$th embedded method, respectively, at time $t_{n+1}$, for $i=2,\ldots, \ell$. Using these equations we obtain
    %     % \begin{align}
    %     %     \Delta t d_{1}^{n} = u^{n+1}-u^{n} =   u(t_{n+1}) - u(t_{n}) + \mathcal{O}(\Delta t^{p+1}) = \mathcal{O}(\Delta t^{}) 
    %     % \end{align}
    % \end{proof}


	\section{Numerical ODE Examples} \label{sec:numerical}
    This section illustrates the effects of multiple relaxation RK methods on several problems with multiple invariants. The following numerical schemes with embedded methods are used in the numerical experiments.
    
    \begin{itemize}
        \item SSPRK(2,2): Two-stage, second-order SSP method \cite{shu1988efficient} with a first-order embedded method (appendix~\ref{app:butcherTableau}).
        \item SSPRK(3,3): Three-stage, third-order SSP method \cite{shu1988efficient} with second-order embedded methods (appendix~\ref{app:butcherTableau}).
        \item Heun(3,3): Three-stage, third-order Heun's method \cite{heun1900neue} with a second-order embedded method (appendix~\ref{app:butcherTableau}).
        \item RK(4,4): Classical four-stage, fourth-order method with a second-order embedded method (appendix~\ref{app:butcherTableau}).
        \item Fehlberg(6,4): Six-stage, fourth-order Fehlberg's method \cite{fehlberg1969low} with third-order embedded methods (appendix~\ref{app:butcherTableau}).
        \item Fehlberg(6,5): Six-stage, fifth-order Fehlberg's method with a fourth-order embedded method \cite{fehlberg1969low}.
        \item DP(7,5): Seven-stage, fifth-order method \cite{prince1981high} with fourth-order embedded methods (appendix~\ref{app:butcherTableau}).
        \item ARK3(2)4L[2]SA: Four-stage, third-order additive Runge-Kutta (ARK) method \cite[Appendix C]{kennedy2003additive} with a second-order embedded ARK method \cite[Appendix C]{kennedy2003additive}. 
        \item ARK4(3)6L[2]SA: Six-stage, fourth-order ARK method \cite[Appendix C]{kennedy2003additive} with a third-order embedded ARK method \cite[Appendix C]{kennedy2003additive}.
    \end{itemize}
    Given a set of embedded RK methods, the multiple relaxation RK method defined in \eqref{modified_Update_rule} requires solving a small system of nonlinear equations for the relaxation parameters at each time step. We use the general nonlinear solver \verb|scipy.optimize.fsolve | to solve the nonlinear system for most of the numerical examples below. In some cases, a combination of optimizers \verb|scipy.optimize.brute| and \verb|scipy.optimize.fmin| is used to find the best solution for the relaxation parameters. The update rule \eqref{modified_Update_rule} for the multiple relaxation RK method, unlike in \eqref{RRK_methods_1}, uses $u^{n+1}$ instead of $u^{n}$, which is observed to provide better robustness in finding the relaxation parameters.
    \subsection{Rigid Body Rotation}
    Consider the system of Euler equations that describes the motion of a free rigid body with its center of mass at the origin, in terms of its angular momenta:
    \begin{subequations}\label{Eq:Euler_equations}
        \begin{align}
            &\dot{u}_{1}=(\alpha - \beta)u_2u_3 \\
            &\dot{u}_{2}=(1-\alpha)u_3u_1  \\
            &\dot{u}_{3}=(\beta-1)u_1u_2 \;,
        \end{align}
    \end{subequations}
    with $\left(u_1(0),u_2(0),u_3(0)\right)^T = (0,1,1)^T$, $\alpha = 1 + \frac{1}{\sqrt{1.51}}$, and $\beta = 1 - \frac{0.51}{\sqrt{1.51}}$. The exact solution is
    \begin{align}
        \left(u_1(t),u_2(t),u_3(t)\right)^T = \left(\sqrt{1.51} \  \textrm{sn}(t,0.51),\textrm{cn}(t,0.51),\textrm{dn}(t,0.51)\right)^T \;,
    \end{align}
    where $\textrm{sn},\ \textrm{cn},\ \text{and} \ \textrm{dn}$ are the elliptic Jacobi functions. This problem has two quadratic conserved quantities:
    \begin{subequations}\label{Eq:Euler_invariantas}
       \begin{align}
            & G_1(u_{1},u_{2},u_{3}) = u_{1}^{2}+ u_{2}^{2}+u_{3}^{2} \;, \\
            & G_2(u_{1},u_{2},u_{3}) = u_{1}^{2}+ \beta u_{2}^{2}+\alpha u_{3}^{2} \;.
        \end{align}
    \end{subequations}
    Here $G_{2}$ is the kinetic energy of the body. First, we present the convergence results obtained with different RK and relaxation methods to confirm that relaxation with multiple invariants also produces the desired order of convergence. Using four different RK schemes (SSPRK(2,2), Heun(3,3), RK(4,4), and DP(7,5)) and their multiple relaxation versions, we solve the system to a final time of $5$ and report the convergence results in Figure ~\ref{fig:EE_Error_Convergence}.
    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Baseline_Mthds_ErrorConv_tf5.pdf}
         \caption{Baseline methods.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Relaxation_Mthds_ErrorConv_tf5.pdf}
         \caption{Multiple relaxation RK methods.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Convergence of numerical solution by different RK methods and their multiple relaxation versions for rigid body rotation \eqref{Eq:Euler_equations}.}
    	\label{fig:EE_Error_Convergence}
    \end{figure}

    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Heuns3p3_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{Heun(3,3) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Fehlbergs6p4_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{Fehlberg(6,4) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_DP5s7p5_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{DP(7,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Changes in invariant \eqref{Eq:Euler_invariantas} obtained with different methods for rigid body rotation \eqref{Eq:Euler_equations}.}
    	\label{fig:EE_Evolution_conserved_quantities}
    \end{figure}
    
    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Heuns3p3_ErrorVsTime_dt1e-01_tf1000.eps}
         \caption{Heun(3,3) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Fehlbergs6p4_ErrorVsTime_dt1e-01_tf1000.eps}
         \caption{Fehlberg(6,4) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_DP5s7p5_ErrorVsTime_dt1e-01_tf1000.eps}
          \caption{DP(7,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time for rigid body rotation \eqref{Eq:Euler_equations}.}
    	\label{fig:EE_error_growth}
    \end{figure}
    Next, we study the error in invariants and the error growth over time by various methods. We integrate the problem with three explicit RK methods and their multiple relaxation versions, Heun(3,3), Fehlberg(6,4), and DP(7,5), with $\Delta t = 0.1$ for all the methods. Figure ~\ref{fig:EE_Evolution_conserved_quantities} plots the error in conserved quantities, confirming that all the relaxation methods preserve both invariants. The solution error growth by all the methods is plotted in Figure ~\ref{fig:EE_error_growth}, which shows a linear error growth when the two invariants are preserved by the relaxation methods. In contrast, the baseline methods produce errors that increase quadratically.

    \subsection{Bi-Hamitonian 3D Lotka-Volterra Systems}
    Next, we consider an ecological predator-prey model of the Lotka-Volterra systems in $3$D, whose equations are given as
    \begin{subequations}\label{Eq:3D_LVS}
        \begin{align}
            &\dot{u}_{1}=u_{1}\left(c u_{2}+u_{3}+\lambda\right) \\
            &\dot{u}_{2}=u_{2}\left(u_{1}+a u_{3}+\mu\right) \\
            &\dot{u}_{3}=u_{3}\left(b u_{1}+u_{2}+\nu\right) \;,
        \end{align}
    \end{subequations}
    where $\lambda, \mu, \nu >0$, $abc=-1$ and $\nu = \mu b - \lambda ab$. We study this problem on the interval $[0,400]$ with parameters $(a,b,c,\lambda,\mu,\nu) = (-1,-1,-1,0,1,-1)$ and the initial condition is taken as $\left(u_1(0),u_2(0),u_3(0)\right)^T = (1,1.9,0.5)^T$. This system has periodic solutions and possesses two nonlinear conserved quantities, known as Casimirs of some skew-symmetric Poisson matrices \cite{ionescu2015geometrical,uzunca2019preservation}:
        \begin{subequations} \label{Eq:3D_LVS_invariants}
            \begin{align}
            & H_1 = ab \ln{u_1} - b \ln{u_2} + \ln{u_3} \;, \\
            & H_2 = ab u_1 + u_2 - a u_3 + \nu \ln{u_2} - \mu \ln{u_3}.
        \end{align}
    \end{subequations}
    
    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Heuns3p3_InvariantVsTime_dt4e-02_tf400.eps}
         \caption{Third order Heun's method, $\Delta t = 0.04$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_RKs4p4_InvariantVsTime_dt1e-01_tf400.eps}
         \caption{Classical fourth order RK method , $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Fehlbergs6p4_InvariantVsTime_dt1e-01_tf400.eps}
         \caption{Fifth order method of Fehlberg, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Changes in invariant \eqref{Eq:3D_LVS_invariants} obtained with different methods for a bi-Hamiltonian $3$D Lotka-Volterra system \eqref{Eq:3D_LVS}.}
    	\label{fig:3DLVS_Evolution_conserved_quantities}
    \end{figure}
    We apply Heun(3,3) with $\Delta t = 0.04$, RK(4,4) with $\Delta t = 0.1$, and DP(7,5) with $\Delta t = 0.1$ to solve the system with and without multiple relaxation. All baseline and multiple relaxation methods preserve the periodicity of the solution. The errors in invariants are shown in Figure ~\ref{fig:3DLVS_Evolution_conserved_quantities}, and we can see that all the multiple relaxation methods preserve the nonlinear invariants for the system over a long time. 
    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Heuns3p3_ErrorVsTime_dt4e-02_tf400.eps}
         \caption{Heun(3,3) with $\Delta t = 0.04$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_RKs4p4_ErrorVsTime_dt1e-01_tf400.eps}
         \caption{RK(4,4) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Fehlbergs6p4_ErrorVsTime_dt1e-01_tf400.eps}
          \caption{Fehlberg(6,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time for a bi-Hamiltonian $3$D Lotka-Volterra system \eqref{Eq:3D_LVS}.}
    	\label{fig:3DLVS_error_growth}
    \end{figure}
    As the closed form of the analytical solution of this system is not known, as a proxy for the exact solution we use the dense output of the Python interface class \verb|scipy.integrate.ode| with \verb|dopri5| method with minimal values for the relative and absolute tolerances. We measure the error in the maximum norm and plot the error over time in Figure ~\ref{fig:3DLVS_error_growth}. The invariant-preserving multiple relaxation methods show asymptotically linear error growth and eventually win in solution accuracy over the quadratically increasing errors of the corresponding baseline methods. 
    
    \subsection{Kepler's Problem}
    \subsubsection{Kepler's Two-Body Problem with Three Invariants}
    So far, each of the numerical examples considered above involves two conserved quantities. We now study Kepler's Two-Body problem with three invariants to demonstrate that the relaxation process can conserve more than two invariants for a system. With one of the two bodies fixed at the center of the $2$D plane, the motion of the other body with position $q = (q_{1},q_{2})$ and momentum $p = (p_{1},p_{2})$ is given by the following system of first order differential equations
    \begin{subequations}\label{Eq:Kepler_two_body_problem}
        \begin{align}
            \dot{q_{1}} & = p_{1} \\
            \dot{q_{2}} & = p_{2} \\
            \dot{p_{1}} & = -\frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} \\
            \dot{p_{2}} & =-\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} \;.
        \end{align}
    \end{subequations}
    Three conserved quantities for Kepler's Two-Body system that we consider for our numerical studies are
    \begin{subequations} \label{Eq:Kepler_invariants}
        \begin{align}
            H(q,p) & = \frac{1}{2}\left(p_{1}^2+p_{2}^2\right)-\frac{1}{\sqrt{q_{1}^2+q_{2}^2}} \ (\text{Hamiltonian}) \;, \\
        	L(q,p) & = q_{1}p_{2}-q_{2}p_{1}\ (\text{angular momentum}) \;, \\
        	A(q,p) & = ||V||_2 \;,
        \end{align}
    \end{subequations}
   where in the last invariant, the well-known Laplace–Runge–Lenz vector function $V$ \cite[Page 26]{haier2006geometric} is defined as 
  \begin{align}
        V & = \begin{bmatrix}
        p_{1} \\
        p_{2} \\
        0
        \end{bmatrix} \times \begin{bmatrix}
        0 \\
        0 \\
        q_{1} p_{2}-q_{2} p_{1}
        \end{bmatrix}-\frac{1}{\sqrt{q_{1}^{2}+q_{2}^{2}}} \begin{bmatrix}
        q_{1} \\
        q_{2} \\
        0
        \end{bmatrix}\;.
   \end{align}
    We consider the Two-Body problem with initial condition $$ \left(q_{1}(0),q_{2}(0),p_{1}(0),p_{2}(0)\right)^{T}=\left(1-e,0,0,\sqrt{\frac{1+e}{1-e}}\right)^{T}$$ with $e=0.5$, and study the conservation of invariants \eqref{Eq:Kepler_invariants} and the global error. Three explicit methods, SSPRK(3,3) with $\Delta t = 0.005$, Fehlberg(6,4) with $\Delta t = 0.05$, and DP(7,5) with $\Delta t = 0.1$ are used as baseline methods to solve the problem.
   \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_SSPRKs3p3_InvariantVsTime_dt5e-03_tf200.eps}
         \caption{SSPRK(3,3) with $\Delta t = 0.005$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_Fehlbergs6p4_InvariantVsTime_dt5e-02_tf200.eps}
         \caption{Fehlberg(6,4) with $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_DP5s7p5_InvariantVsTime_dt1e-01_tf200.eps}
         \caption{DP(7,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Change in conserved quantities \eqref{Eq:Kepler_invariants} obtained with different methods for Kepler's Two-Body problem \eqref{Eq:Kepler_two_body_problem}.}
    	\label{fig:Kepler_Evolution_conserved_quantities}
    \end{figure}
     
    \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_SSPRKs3p3_ErrorVsTime_dt5e-03_tf200.eps}
         \caption{SSPRK(3,3) with $\Delta t = 0.005$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_Fehlbergs6p4_ErrorVsTime_dt5e-02_tf200.eps}
         \caption{Fehlberg(6,4) with $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_DP5s7p5_ErrorVsTime_dt1e-01_tf200.eps}
          \caption{DP(7,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time for Kepler's Two-Body problem \eqref{Eq:Kepler_two_body_problem}.}
    	\label{fig:Kepler_error_growth}
    \end{figure}
    Together with the baseline methods, the relaxation versions of these methods now require two more "independent" embedded methods to solve the system as it has three conserved quantities. The new embedded methods are provided in the appendix ~\ref{app:butcherTableau}, each having order of accuracy one less than that of the corresponding baseline method. Figure ~\ref{fig:Kepler_Evolution_conserved_quantities} demonstrates the advantage of relaxation over baseline RK methods. All the relaxation methods conserve three quantities almost to machine precision, while the baseline RK methods conserve them to around four decimal places. The consequence of these results is reflected in the asymptotic error growth by these methods, shown in Figure ~\ref{fig:Kepler_error_growth}. It shows a quadratic error growth by the baseline methods, while the corresponding multiple relaxation methods achieve a linear error growth over a long time.
    
    \subsubsection{Perturbed Kepler's Problem}
    The governing equations of the perturbed Kepler's problem \cite{haier2006geometric} are given by the following system
    \begin{subequations}\label{Eq:Perturbed_Kepler_problem}
        \begin{align}
            \dot{q_{1}} & = p_{1} \\
            \dot{q_{2}} & = p_{2} \\
            \dot{p_{1}} & = -\frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} -\mu \frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{5/2}} \\
            \dot{p_{2}} & =-\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}}  -\mu\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{5/2}} \;,
        \end{align}
    \end{subequations}
    where $\mu$ is a small number taken as $0.005$ for our numerical studies. Previous studies of this problem show that it is important for a numerical method to preserve both the invariants
    \begin{subequations} \label{Eq:Perturbed_Kepler_invariants}
        \begin{align}
            H(q,p) & = \frac{1}{2}\left(p_{1}^2+p_{2}^2\right)-\frac{1}{\sqrt{q_{1}^2+q_{2}^2}}-\frac{\mu}{2\sqrt{\left(q_{1}^2+q_{2}^2\right)^3}}\ (\text{Hamiltonian}) \;, \\
        	L(q,p) & = q_{1}p_{2}-q_{2}p_{1}\ (\text{angular momentum}) \;,
        \end{align}
    \end{subequations}
    to capture the correct behavior of the solution. With the same initial conditions as in Kepler's two-body problem above but with a different eccentricity $e=0.6$, we solve the system using the baseline and the relaxation versions of the methods SSPRK(3,3) with $\Delta t = 0.03$, Fehlberg(6,4) with $\Delta t = 0.05$, and DP(7,5) with $\Delta t = 0.1$. The analytical solution is not available, so we instead use the dense output of Python interface class \verb|scipy.integrate.ode| with \verb|dopri5| method with the relative and absolute tolerances both equal to $10^{-16}$. The errors in both invariants and the numerical solutions of the orbits are presented in Figure ~\ref{fig:Perturbed_Kepler_Evolution_conserved_quantities} and Figure ~\ref{fig:Per_Kepler_error_growth}, respectively.

  \begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_SSPRKs3p3_InvariantVsTime_dt5e-02_tf300.eps}
        \caption{SSPRK(3,3) with $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Fehlbergs6p4_InvariantVsTime_dt5e-02_tf300.eps}
        \caption{Fehlberg(6,4) with $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_DP5s7p5_InvariantVsTime_dt1e-01_tf300.eps}
        \caption{DP(7,5) with $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
        \caption{Changes in conserved quantities \eqref{Eq:Perturbed_Kepler_invariants} by different methods for perturbed Kepler's problem \eqref{Eq:Perturbed_Kepler_problem}.}
        \label{fig:Perturbed_Kepler_Evolution_conserved_quantities}
    \end{figure}
    
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_SSPRKs3p3_Sol_dt5e-02_tf300.eps}
        %\caption{Third order method of Shu \& Osher, $\Delta t = 0.03$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_Fehlbergs6p4_Sol_dt5e-02_tf300.eps}
        %\caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_DP5s7p5_Sol_dt1e-01_tf300.eps}
        %\caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_SSPRKs3p3_Sol_dt5e-02_tf300.eps}
        %\caption{Third order method of Shu \& Osher, $\Delta t = 0.03$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_Fehlbergs6p4_Sol_dt5e-02_tf300.eps}
        %\caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_DP5s7p5_Sol_dt1e-01_tf300.eps}
        %\caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_SSPRKs3p3_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Fehlbergs6p4_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_DP5s7p5_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Exact_Orbit_dt3e-02_tf300.eps}
    \end{subfigure}
    	\caption{Solution of perturbed Kepler's problem \eqref{Eq:Perturbed_Kepler_problem} by different methods. The first three plots in the last row of the figure compare the body's position by different methods at the few last steps of the simulation.}
    	\label{fig:Perturbed_Kepler_Solutions}
    \end{figure}
     Figure ~\ref{fig:Perturbed_Kepler_Evolution_conserved_quantities} shows that, in contrast with the underlying baseline methods, all the relaxation methods preserve the invariants up to the machine precision and correctly produce the elliptic orbit that precesses slowly around one of its foci (Figure ~\ref{fig:Perturbed_Kepler_Solutions}). Note that the effect of preserving the conserved quantities is only noticeable for the third-order method, where the baseline third-order method incorrectly captures the motion of orbits. Even though visually, the higher-order methods appear to produce the correct behavior of the trajectories without relaxation, in truth, these methods give completely wrong positions as time grows. As can be seen in Figure ~\ref{fig:Per_Kepler_error_growth}, the error of the baseline method increases quadratically with time until it reaches a saturation point of $100$\% error, leading to incorrect orbits of the body. The invariant-preserving relaxation approach, in contrast, results in a linear accumulation of error over time, which leads to a significantly smaller error, producing correct orbits of the body for a long time. 
     
     \begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_SSPRKs3p3_ErrorVsTime_dt5e-02_tf300.eps}
         \caption{SSPRK(3,3) with $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_Fehlbergs6p4_ErrorVsTime_dt5e-02_tf300.eps}
         \caption{Fehlberg(6,4) with $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_DP5s7p5_ErrorVsTime_dt1e-01_tf300.eps}
          \caption{DP(7,5) with $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time for perturbed Kepler's problem \eqref{Eq:Perturbed_Kepler_problem}.}
    	\label{fig:Per_Kepler_error_growth}
    \end{figure}

    \section{Application to the Korteweg–De Vries (KdV) equation}
    Finally we consider a PDE example; namely,
    the Kortweg-de Vries (KdV) equation
    \begin{align}\label{KdV_Equation}
        u_t+6uu_x+u_{xxx} & = 0, \ \text{on} \ [x_{L},x_{R}]\times(0,T] \;,
    \end{align}
    with periodic boundary condition $u(x_L,t) = u(x_R,t)$.
    The KdV equation has infinitely many conserved quantities, of which the first three are
        \begin{subequations} \label{KdV_invariants}
        \begin{align}
            \int u \ dx \ (\text{mass}) \\
        	\int \frac{1}{2} u^2 \ dx \ (\text{energy}) \\
        	\int \left(2u^3 -u_x^2  \right) dx \ (\text{Whitham}) \;.
        \end{align}
    \end{subequations}
    It has been shown that, for the case of a 1-soliton solution, numerical methods that conserve both mass and energy give solutions whose error grows linearly in time, whereas methods that don't conserve these quantities generically yield quadratic error growth \cite{de1997accuracy}.
    In the same work, preliminary experiments with conservative methods applied to two interacting solitons also exhibited linear error growth, except during the soliton interaction.  However, there are no theoretical results except in the 1-soliton case.

    In this section we investigate the effect of conserving only the mass (which is conserved automatically by even the baseline RK methods) versus using relaxation to conserve both mass and energy, or  all three invariants \eqref{KdV_invariants}.  We consider initial data with one, two, or three solitons.
    We use relaxation to enforce the conservation of the nonlinear invariants.

    To discretize in space, we introduce an evenly-spaced grid ${x_i}$ with $x_1=x_L$ and $x_N=x_R-\Delta x$.
    We enforce semi-discrete mass and energy conservation by employing the split form spatial discretization \cite{ranocha2006broad}
    \begin{equation}\label{SBP_semi_discretization}
       \partial_{t} U+6 \times \frac{1}{3}\left(D_{1}(U \cdot U)+U \cdot\left(D_{1} U\right)\right)+D_{3} U=0,
    \end{equation}
    where $D_1, D_3$ are skew-symmetric differentiation matrices approximating the first- and third-derivative operators, respectively (here we use Fourier spectral differentiation matrices),
    and $U_i(t) \approx u(x_i,t)$.  
    In \eqref{SBP_semi_discretization} the dot $\cdot$ denotes element-wise multiplication.
    This guarantees semi-discrete conservation of the discrete mass and energy
        \begin{subequations} \label{KdV_discrete_inv_mass_energy}
        \begin{align}
            \eta_0 & := \Delta x \sum_{j}U_j \\
            \eta_1 & := \Delta x \sum_{j}|U_j|^2,
        \end{align}
    \end{subequations}
    (up to rounding errors), regardless of the grid spacing $\Delta x$.  However, the third invariant is conserved only to the level of the spatial truncation error.  This can be made small by using a fine grid, and will be discussed further in Section \ref{sec:conserve3}.

    The semi-discretization \eqref{SBP_semi_discretization} is stiff, since $\|D_3\| = {\mathcal O}(\Delta x^{-3})$.  We therefore make use of IMEX RK schemes in time, handling the stiff linear term implicitly and the nonlinear term explicitly.  We use two IMEX schemes from \cite[Appendix C]{kennedy2003additive}, which were introduced already at the beginning of Section \ref{sec:numerical}.
    
    \subsection{Conservation of mass and energy}
    In this section we investigate how the conservation of mass and energy affects the temporal error growth, relative to methods that conserve only the mass.  We consider 3 different initial conditions, consisting of one, two, or three solitons, as detailed in Appendix \ref{app:soliton-solutions}.

    \subsubsection{One soliton}
    We first consider the 1-soliton solution ((a) in appendix \ref{app:soliton-solutions}) on the domain $[x_{L},x_{R}]=[-20,60]$ of length $L = 80$ and $N=512$ spatial grid points and integrate from $t=0$ to $t=20$. Table ~\ref{Table:1_invariant_error} displays the 
    maximum deviation of each invariant compared to its initial value, confirming that mass is conserved in all cases, while energy is conserved only by the relaxation methods.
    In Figure ~\ref{fig:KdV_1_sol_1_inv_GlobalErrors}, we plot the global error as a function of time. The errors behave linearly for RK methods with relaxation and quadratically without relaxation. These numerical results agree with the analytical results presented in \cite{de1997accuracy}, i.e., in the case of 1-soliton solution of the KdV equation, the errors incurred by methods conserving mass and energy grow linearly as opposed to quadratic growth by non-conservative methods.
    \begin{table}
    \centering
    \begin{tabular}{ | c | l | c | c | c |}
        \hline
               &    &          \multicolumn{3}{c|}{Invariant Error in}\\
        \hline
        Case & Methods & Mass & Energy & Whitham  \\
        \hline
        \multirow{4}*{1-soliton and 1 invariant} & Baseline ImEx (3,2)  & $1.18e-13$ & $5.38e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $1.19e-13$ & $2.22e-16$ &  \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $1.04e-13$ & $1.05e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $1.06e-13$ & $3.33e-16$ &  \\
        \hline
        \multirow{4}*{2-soliton with 1 invariant} & Baseline ImEx (3,2)  & $9.50e-14$ & $1.10e-01$ & \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $8.97e-14$ & $4.44e-16$ & \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $5.68e-14$ & $2.32e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $5.86e-14$ & $8.88e-16$ &  \\
        \hline 
        % \multirow{4}*{2-soliton with 2 invariants} & Baseline ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Baseline ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \hline 
        \multirow{4}*{3-soliton with 1 invariant} & Baseline ImEx (3,2)  & $6.57e-14$ & $2.07e-01$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $7.19e-14$ & $2.22e-16$ &  \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $3.82e-14$ & $4.62e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $3.73e-14$ & $8.88e-16$ &  \\
        \hline
        % \multirow{4}*{3-soliton with 2 invariants} & Baseline ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Baseline ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \hline 
    \end{tabular}
    \caption{Maximum invariant errors by various methods for different n-solitons with 1 invariant case.}
    \label{Table:1_invariant_error}
    \end{table}
     
    %  \begin{table} \small%
    %     \begin{tabular}{| c | c | c | c | c |}
    %     \hline
    %     Case & Methods & Mass & Energy & Whitham  \\
    %     \hline
    %     \cline{2-4}
    %                      & Second solution & Data 1 & Yes \\
    %                      &                & Data 2 &  \\
    %                      &                & Data 3 &  \\
    %     \hline
    %     \end{tabular}
    % \end{table}
    
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_1_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf20.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_1_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf20.eps}
    \end{subfigure}
	\caption{Error growth over time for a 1-soliton solution of the KdV equation.  Relaxation is used to enforce conservation of $\eta_1$.  Red dotted line: baseline IMEX method, i.e., IMEX method without relaxation and solid green line: IMEX method with relaxation.  For all cases, $\Delta t = 0.1$.}
	\label{fig:KdV_1_sol_1_inv_GlobalErrors}
    \end{figure}
    
    \subsubsection{Two solitons}
    Next, we consider a 2-soliton solution over the region $[x_{L},x_{R}]=[-80,80]$ and use the semi-discretization \eqref{SBP_semi_discretization} with $N=768$ spatial grid points, integrating from $t=-25$ to $t=25$. 
    The error growth for the resulting solutions is presented in Figure ~\ref{fig:KdV_2_sol_1_inv_GlobalErrors}.  In this case, there are no available theoretical results to guarantee the error growth of conservative methods will be better than for non-conservative methods.  For the two relaxation methods employed here we see markedly different behaviors; one method exhibits sublinear growth, while the other exhibits something between linear and quadratic growth at long times.  In both cases, the conservative (relaxation) methods provide solutions that are drastically more accurate compared to the non-conservative counterparts, which exhibit the expected quadratic error growth.  All methods exhibit a dip in the error during the soliton interaction, as was observed in \cite{de1997accuracy}.
     \abhi{How do we explain such error growth behavior for the 2-soliton 1-invariant case?} 
     
     \subsubsection{Three solitons}
     Finally, we consider the case of a 3-soliton solution on the domain $[x_{L},x_{R}]=[-130,130]$ with $N=1024$ spatial grid points, integrated from $t=-50$ to $t=50$. Figure ~\ref{fig:KdV_3_sol_1_inv_GlobalErrors} shows the errors over time. In this case, the conservative (relaxation) approach results in quadratic growth of errors similar to baseline IMEX methods, although the conservative solutions still have much smaller errors.  We examined the structure of the errors in this case and found that although the total energy is conserved, the energy of individual solitons changes linearly over time, leading to  quadratically growing phase errors for all three solitons.  It is unclear why the 2-soliton case does not exhibit a similar effect.
     
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf25.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf25.eps}
    \end{subfigure}
	\caption{Error growth over time for a 2-soliton solution of the KdV equation.  Relaxation is used to enforce conservation of $\eta_1$.  Red dotted line: baseline IMEX method, i.e., IMEX method without relaxation and solid green line: IMEX method with relaxation.  For all cases, $\Delta t = 0.1$.}
	\label{fig:KdV_2_sol_1_inv_GlobalErrors}
    \end{figure}
    
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf50.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf50.eps}
    \end{subfigure}
	\caption{Error growth over time for a 3-soliton solution of the KdV equation.  Relaxation is used to enforce conservation of $\eta_1$. Red dotted line: baseline IMEX method, i.e., IMEX method without relaxation and solid green line: IMEX method with relaxation.  In all cases, $\Delta t = 0.1$.}
	\label{fig:KdV_3_sol_1_inv_GlobalErrors}
    \end{figure}
   
     \subsection{Multiple relaxation: attempting to restore conservation through relaxation}\label{sec:conserve3}
    We have seen that conserving only two invariant quantities (mass and energy) is not generally sufficient to produce linear error growth for the 2- and 3-soliton solutions.  It is natural to ask whether conserving a third invariant will improve this. Since we do not have a semi-discretization that preserves discrete analogs of all three invariants simultaneously, we instead attempt to use a sufficiently fine spatial grid so as to minimize the spatial truncation errors altogether.  We introduce the discrete approximation
    \begin{align}
        \eta_2 := \text{fill in}
    \end{align}
    and test how well this quantity is conserved (using non-conservative time integration) as we refine the spatial grid.  
    %employ the same pseudospectral spatial discretization as in \eqref{SBP_semi_discretization}. With this semi-discretized system, we compute the Whitham's invariant using the composite Simpson rule, in which the first derivative is calculated using the discrete Fourier transform. The composite Simpson rule is used to calculate the values of Whitham's invariant to accurately capture the errors in this conserved quantity, which is crucial, especially for the relaxation approach. We choose the number of spatial grid points so that no further error reduction can be obtained in the time derivative of Whitham's invariant by taking more grid points. 
    This leads to a choice of $N = 1024$ grid points for a 2-soliton solution on the domain $[-80,80]$ and $N = 1536$ grid points for a 3-soliton solution on the domain $[-130,130]$. %This allows us to study the error behavior solely by the time-stepping methods.
    
    \subsubsection{Solution of the relaxation equations for a non-conservative system}
    \emph{We need to present some indication of how close we are to semi-discrete conservation.}
    Since $\eta_2$ is not exactly conserved by the true semi-discrete solution, we have no theoretical guarantee of the existence of a solution of the relaxation equations \eqref{relaxation-equations}.  In fact, this represents an interesting potential application of the relaxation technique -- if conservation is lost in the process of semi-discretization, can we restore it through time discretization, and what effect will that have?  The results below represent a first exploration of this question, which might serve as a starting point for further work.

    We find that at many timesteps, the `fsolve` routine from `scipy.optimize` gives a solution
    accurate to significantly less than double precision, consistent with our estimates of the accuracy of conservation for the semi-discrete scheme.  In order to ensure that we obtain the most accurate solution possible, we do an additional search using numerical optimization routines from `scipy.optimize` when the solution from `fsolve` is inaccurate.
    %Like all the examples above, we also use the python 'fsolve' to find the solution for the relaxation parameters at each step of our numerical method. We observe that the 'fsolve' method fails to find a solution to the invariant equations at many steps in our numerical simulation. In these cases, we further use the Python 'brute' method to find a good initial guess for the Python 'fmin' method and find a solution for relaxation parameters that minimizes the sum of squares of the invariant equations. Finally, we choose the solution with a better residual error among the two solutions given by the two methods.

    \subsubsection{Results}
    Figures ~\ref{fig:KdV_2_sol_2_inv_InvariantErrors} and ~\ref{fig:KdV_3_sol_2_inv_InvariantErrors} show the deviation of the invariants over time for the 2-soliton and 3-soliton cases, respectively.  Relaxation methods improve the error in invariants, but they are not up to the machine accuracy.

        \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK32_InvariantVsTime_dt1e-02_tf25.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK43_InvariantVsTime_dt1e-02_tf25.eps}
    \end{subfigure}
	\caption{Deviation of each invariant from its initial value for a 2-soliton solution of the KdV equation.  Relaxation is used to (attempt to) enforce conservation of $\eta_1$ and $\eta_2$.  In all cases, $\Delta t = 0.01$.}
	\label{fig:KdV_2_sol_2_inv_InvariantErrors}
    \end{figure}

    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK32_InvariantVsTime_dt1e-02_tf50.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK43_InvariantVsTime_dt1e-02_tf50.eps}
    \end{subfigure}
	\caption{Deviation of each invariant from its initial value for a 3-soliton solution of the KdV equation.  Relaxation is used to (attempt to) enforce conservation of $\eta_1$ and $\eta_2$.  In all cases, $\Delta t = 0.01$.}
	\label{fig:KdV_3_sol_2_inv_InvariantErrors}
    \end{figure}
    The error growth behavior for these examples is plotted in Figures \ref{fig:KdV_2_sol_2_inv_GlobalErrors} and \ref{fig:KdV_3_sol_2_inv_GlobalErrors}.  We observe that relaxation may yield no improvement or even degrade the accuracy of the solution over short times, but provides a noticeable improvement in accuracy over sufficiently long times.  Interestingly, we observe roughly linear error growth at long times, although there is significant jitter, probably due to the lack of an exact solution to the relaxation equations.
    
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK32_ErrorVsTime_dt1e-02_tf25.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK43_ErrorVsTime_dt1e-02_tf25.eps}
    \end{subfigure}
	\caption{Error growth over time for a 2-soliton solution of the KdV equation.  Relaxation is used to enforce conservation of $\eta_1$ and $\eta_2$ as nearly as possible. Red dotted line: baseline IMEX method, i.e., IMEX method without relaxation and solid green line: IMEX method with relaxation.  In all cases, $\Delta t = 0.01$.}
	\label{fig:KdV_2_sol_2_inv_GlobalErrors}
    \end{figure}

    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK32_ErrorVsTime_dt1e-02_tf50.eps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK43_ErrorVsTime_dt1e-02_tf50.eps}
    \end{subfigure}
	\caption{Error growth over time for a 3-soliton solution of the KdV equation.  Relaxation is used to enforce conservation of $\eta_1$ and $\eta_2$ as nearly as possible. Red dotted line: baseline IMEX method, i.e., IMEX method without relaxation and solid green line: IMEX method with relaxation.  In all cases, $\Delta t = 0.01$.}
	\label{fig:KdV_3_sol_2_inv_GlobalErrors}
    \end{figure}


   
\section{Conclusions}
    In this work, we propose a generalization of the relaxation framework for RK methods to preserve multiple nonlinear conserved quantities of a dynamical system. We prove the existence of the relaxation parameters and the accuracy of the generalized relaxation methods under some conditions. Depending on the system's stiffness, the generalized relaxation approach is applied with different RK methods, such as explicit RK and additive RK methods. Numerical results demonstrate that the generalized relaxation RK methods can conserve multiple conserved quantities and produce qualitatively better numerical solutions. 

    An important case study of our numerical experiments includes the KdV equation with multi-soliton solutions. With a conservative semi-discretization of the KdV equation preserving mass and energy, the relaxation approach applied with ARK methods successfully preserves the invariants for 1, 2, and 3-soliton solutions. We observe that mass and energy preservation do not produce linear error growth for multi-soliton solutions for the KdV equation. Some numerical results applying relaxation methods to a non-conservative semi-discretization (enforcing conservation of a third nonlinear invariant ) of the KdV equation are presented. Numerical results suggest that relaxation methods can be advantageous if we are interested in long time numerical solutions. 

    The application of this general relaxation framework to the nonlinear Schr\"{o}dinger equation with multiple nonlinear invariants is a subject of ongoing research. Another possible research direction is extending the generalized relaxation approach framework to the other class of time integration schemes, such as linear multistep methods, and improving the underlying methods' numerical performance.
%================================================================================
\appendix
%================================================================================
\section{List of RK Methods} 
\label{app:butcherTableau}
%================================================================================

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{2.5cm}{!}{%
    	\begin{tabular}{l|l l}
             0  &    0 \\                        
             1  &    1  &   0  \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/2  &   1/2 \\
             \hline
            $\vec{b}^{\,2}$  &   1/3  &   2/3	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{SSPRK(2,2): Second-order method $(A,\vec{b}^{\,1})$ with a first-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_ssprk22}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{10cm}{!}{%
    	\begin{tabular}{l|l l l}
             0  &    0 \\                        
             1  &    1  &   0  \\ 
             1/2 &          1/4   &        1/4 & 0 \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/6  &          1/6    &        2/3   \\
             \hline
            $\vec{b}^{\,2}$  &   0.291485418878409 & 0.291485418878409 & 0.417029162243181	\\
            \hline
            $\vec{b}^{\,3}$  & 0.395011932394815 & 0.395011932394815 & 0.209976135210371
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{SSPRK(3,3): Third-order method $(A,\vec{b}^{\,1})$ with $(A,\vec{b}^{\,2})$ and $(A,\vec{b}^{\,3})$ as second-order embedded methods.}
    \label{tab:BT_ssprk33}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{10cm}{!}{%
    	\begin{tabular}{l|l l l}
             0  &    0 \\                        
             1/3  &    1/3  &   0  \\ 
             2/3 &      0   &    2/3 & 0 \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/4  &          0   &        1/4   \\
             \hline
            $\vec{b}^{\,2}$  &   0.006419303047187  & 0.487161393905626 &  0.506419303047187	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{Heun(3,3): Third-order method $(A,\vec{b}^{\,1})$ with a second-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_heun33}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{4cm}{!}{%
    	\begin{tabular}{l|l l l l}
             0  &    0 \\                        
             1/2  &    1/2  &   0  \\ 
             1/2 &      0   &    1/2 & 0 \\ 
             1   &      0   &    0   &     1      &    0  \\
             \hline
            $\vec{b}^{\,1}$  &   1/6   &        1/3    &       1/3      &     1/6  \\
             \hline
            $\vec{b}^{\,2}$  &   1/4   &        1/4      &     1/4     &      1/4	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{RK(4,4): Fourth-order method $(A,\vec{b}^{\,1})$ with a second-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_rk44}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{18cm}{!}{%
    	\begin{tabular}{l|l l l l l l}
             0  &    0 \\                        
             1/4 &          1/4  &          0   \\ 
             3/8 &	3/32 &	9/32 & 0 \\ 
             12/13	& 1932/2197 & 	-7200/2197 &	7296/2197 &   0\\
             	1 &	439/216 &	-8 &	3680/513 &	-845/4104 &    0\\
              1/2 &	-8/27  &	2 &	-3544/2565 &	1859/4104 &	-11/40 &	    0\\
             \hline
             $\vec{b}^{\,1}$  & 16/135	& 0	& 6656/12825& 28561/56430	& -9/50 &	2/55 \\
             \hline
            $\vec{b}^{\,2}$  &  25/216 &	0 &	1408/2565 &	2197/4104  &	-1/5  &	0   \\
             \hline
            $\vec{b}^{\,3}$  &   0.122702088570621 &   0.000000000000003 &  0.251243531398616 & -0.072328563385151 &  0.246714063515406 &  0.451668879900505 \\
            \hline
            $\vec{b}^{\,4}$  & 0.150593325320835 & 0.000000000000003 & 0.275657325006399 & 0.414789231909538 & -0.131467847351019 & 0.290427965114243
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{Fehlberg(6,4): Fifth-order method $(A,\vec{b}^{\,1})$ with a fourth-order embedded method $(A,\vec{b}^{\,2})$ , and $(A,\vec{b}^{\,3})$ and $(A,\vec{b}^{\,4})$ as third-order embedded methods.}
    \label{tab:BT_fehlberg54}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{17cm}{!}{%
    	\begin{tabular}{l|l l l l l l l}
             0  &    0 \\                        
             1/5 &          1/5  &          0   \\ 
            3/10 & 	3/40 & 	9/40 & 0 \\ 
             4/5 & 	44/45 & 	-56/15 & 	32/9 &   0\\
            8/9	&  19372/6561 & 	-25360/2187 & 	64448/6561 & 	-212/729 &    0\\
            1	& 9017/3168  & 	-355/33	 &  46732/5247 & 	49/176 & 	-5103/18656 &	    0\\
            1	&  35/384  & 	0  & 	500/1113  & 	125/192 & 	-2187/6784 & 	11/84  &    0\\
             \hline
            $\vec{b}^{\,1}$  &  35/384 & 	0  & 	500/1113  & 	125/192  & 	-2187/6784  & 	11/84  & 	0   \\
             \hline
            $\vec{b}^{\,2}$  &   5179/57600  & 	0  & 	7571/16695  & 	393/640  & 	-92097/339200  &  187/2100  & 1/40	\\
            \hline
            $\vec{b}^{\,3}$  & 0.159422044716717 & 0.000000000000009 & 0.310936711045800 & 0.444052776789396 & 0.307005319740028 & -0.230738637667449 & 0.009321785375499
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{DP(7,5): Fifth-order method $(A,\vec{b}^{\,1})$ with $(A,\vec{b}^{\,2})$ and $(A,\vec{b}^{\,3})$ as fourth-order embedded methods.}
    \label{tab:BT_dp54}
\end{table}
%================================================================================
\section{Soliton Solutions} 
\label{app:soliton-solutions}
Diffrent soliton solutions \cite{ranocha2020relaxation} of the KdV equation \eqref{KdV_Equation} are given below: 
\begin{enumerate}
    \item [(a)] \textbf{1-soliton solution}:
    \begin{align}
        u(x,t)= \beta_1 \sech ^2(\xi_1) \;,
    \end{align}
    where $\beta_1 = 1$ and $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$.
    \item [(b)] \textbf{2-soliton solution}:
    \begin{align}
        u(x, t) = -\frac{2(\beta_1-\beta_2)\left(\beta_2 \csch^2(\xi_2)+\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)\right)^2} \;,
    \end{align}
    where $\beta_1 = 0.5$, $\beta_2 = 1$, $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$, and $\xi_2 = \frac{\sqrt{\beta_2}(x-2 \beta_2 t)}{\sqrt{2}}$.
    \item [(c)] \textbf{3-soliton solution}:
    \begin{align}
        u(x, t) = \beta_1\sech^2(\xi_1)- \frac{2(\beta_2-\beta_3)\left(\frac{2(\beta_3-\beta_1)\left(\beta_3 \csch^2(\xi_3)-\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_3} \tanh(\xi_3)-\sqrt{2 \beta_1} \tanh(\xi_1)\right)^2}-\frac{2(\beta_1-\beta_2)\left(\beta_2 \csch^2(\xi_2)+\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)\right)^2} \right)}{\left(\frac{2(\beta_1-\beta_2)}{\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)}-\frac{2(\beta_3-\beta_1)}{\sqrt{2 \beta_3} \tanh(\xi_3)-\sqrt{2 \beta_1} \coth(\xi_1)}\right)^2}\;,
    \end{align}
    where $\beta_1 = 0.4$, $\beta_2 = 0.7$, $\beta_3 = 1$, $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$, $\xi_2 = \frac{\sqrt{\beta_2}(x-2 \beta_2 t)}{\sqrt{2}}$, and $\xi_3 = \frac{\sqrt{\beta_3}(x-2 \beta_3 t)}{\sqrt{2}}$.
\end{enumerate}

%================================================================================
%================================================================================
\section*{Acknowledgments}
%================================================================================

%================================================================================




%================================================================================


==> img/article_file_old.tex <==
%===============================================================================
%===============================================================================
\renewcommand{\O}{{\mathcal O}}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}
\newcommand{\vardbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}

\newcommand{\Err}{\mathcal{I}(\zeta)}  
\newcommand{\myremarkend}{$\spadesuit$} 
\newcommand{\lbmap}{\left[} 
\newcommand{\rbmap}{\right]} 
\newcommand{\WSOset}{\mathbb{W}_q}
\newcommand{\OCset}{\mathbb{V}_{p}}
\newcommand{\numc}{n_c}
\newcommand{\minPolc}{P_{\rm C}}
\newcommand{\qso}{\tilde{q}}
\newcommand{\RzCoeff}{\beta}
\newcommand{\Sredr}{\tilde{r}}
\newcommand{\BigO}{{\mathcal{O}}}
\newcommand{\Dt}{\Delta t}
\newcommand{\vecpower}[2]{\vec{#1}^{\,#2}}
\newcommand{\kgen}{m}
\newcommand{\basismat}{L}
\newcommand{\Umat}{U}
\newcommand{\Vmat}{V}
\newcommand{\Wmat}{W}
\newcommand{\bsmall}{\hat{\vec{b}}}
\newcommand{\Ksmall}{\hatK}
\newcommand{\Real}{\mathbb{R}}
%=========================
\newcommand{\kibitz}[2]{\textcolor{#1}{#2}}
\newcommand{\abhi}[1] {\kibitz{red}{[AB says: #1]}}
%=========================
 \abhi{ Novelty statement: Explain the scientific innovations of the paper and how they are aligned with the scope of SISC as expressed in the editorial policy. If building on recently published work, discuss how the paper provides a substantial advance. The novelty statement must explicitly discuss the scientific innovations and must not merely repeat the abstract. Authors may elaborate further in a cover letter to help editors in evaluating the novelty of the contribution}

Runge-Kutta methods are some of the most popular time integrators in many applications. Yet, they can not preserve all nonlinear invariants for a conservative dynamical system, which might lead to non-physical numerical solutions or spurious blow-up of the numerical solutions. A modification of RK methods, known as the relaxation RK methods, was proposed to preserve one nonlinear invariant of a conservative system, which greatly improves the overall quality of the numerical solutions and produce better accurate solution compared to the unmodified RK method. In many applications, conserving one nonlinear invariant of a dynamical system with multiple nonlinear invariants (for example, the KdV equation with multi-soliton solution) is not enough to significantly improve the accuracy over a long time. And it is natural to ask whether one can design or modify the existing methodology to conserve more than one invariant and improve the quality of the numerical solutions. This work uses a set of given embedded RK methods and generalizes the relaxation approach to preserve multiple invariants when applied to a conservative dynamical system. Proof of the accuracy of the modified RK methods is given. Several numerical examples are presented to demonstrate the significance of preserving multiple nonlinear conserved quantities. Numerical results indicate that these modified RK methods can be advantageous in applications where long time accurate numerical solutions are important.


	\section{Introduction}
    The development of structure-preserving time integrators that capture different qualitative properties of initial value problems has been a primary focus of numerical analysis for the last few decades. Here we are interested in conserved quantities preserved by the true solution of a system of differential equations.  Consider an autonomous ordinary differential equation system with an initial condition
    \begin{equation}\label{IVP_1}
             \dot{u}(t)  = f\left(u(t)\right), \  u(0) = u_{0}, \ u(t)\in \Real^{m} \;,
    \end{equation}
    where $ \ f : \mathcal{D} \subset \Real^m \to \Real^m$ is a sufficiently smooth function. We say that the problem \eqref{IVP_1} has $\ell$ conserved quantities defined in terms of a $\mathcal{C}^{1}(\mathcal{\bar{D}})$ function $ \ G: \mathcal{\bar{D}} \subset \Real^{m} \to \Real^{\ell}$ if
    % if the solution $u(t)$ of \eqref{IVP_1} belongs to  $\mathcal{M} := \left\{u\in \Real^m: G(u) = G(u_{0}) \right\}$ and 
    \begin{align*}
        \frac{\textrm{d}}{\textrm{dt}}G(u(t)) = \nabla G(u)^{T}f(u) = 0 \;.
    \end{align*}
    %This $\ell$-invariant function $G$ is also called weak invariant \cite{haier2006geometric} of \eqref{IVP_1} and it depends on initial conditions. A sufficiently smooth scalar function $ \ I: \mathcal{D} \subset \Real^{m} \to \Real$ is called a strong invariant or a first integral if 
    %\begin{align*}
    %    \nabla I(u)^{T}f(u) = 0, \ u \in \mathcal{D}\;.
    %\end{align*}
    %Strong invariants do not depend on the initial conditions and $I(u(t))$ is constant for all solutions $u(t)$ of the differential system. 
    Time-dependent differential equations with multiple conserved quantities (mass, energy, etc.) appear in many applications. Examples include special classes of ordinary differential equations (for example, the Lotka-Volterra system), various Hamiltonian systems (the classic example is Kepler's Two-Body problem), many partial differential equations, including the Korteweg-de Vries (KdV) equation, nonlinear Schrodinger equation, etc. Since in general numerical integrators do not conserve invariants of the systems, in recent years the preservation of invariants has grown in significance as a criterion of a numerical scheme's effectiveness \cite{li1995finite}. Failure to maintain the invariants sometimes leads to non-physical numerical solutions \cite{gear1992invariants} or spurious blow-up of the numerical solutions \cite{arakawa1997computational} when numerically integrating the system. In many cases, conservative schemes are also proved to have better error growth behavior over time than nonconservative methods \cite{de1997accuracy,duran2000numerical}. In such cases, conservative methods may be the only approach that gives acceptable numerical solutions for long-time simulations.  Further studies illustrating the superiority of conservative approaches over generic methods in this regard can be found in \cite{calvo1993development, cano1997error}.
    
    Runge-Kutta methods are among the most widely used time-integration techniques, and it is natural to consider these methods while studying invariant preserving numerical integrators. All Runge-Kutta methods preserve linear invariants.  Only symplectic RK methods preserve quadratic invariants \cite{cooper1987stability}, and such methods must be fully implicit.  It is also well-known \cite{haier2006geometric} that no Runge-Kutta method can preserve all polynomial invariants of degree $n \geq 3$. This restriction motivates the development of new techniques that can preserve conserved quantities, especially the general polynomial invariants. 
    
    Several approaches have been introduced to overcome the shortcomings mentioned above in the existing numerical integrators. For any given differential system with a quadratic invariant, Dekker and Verwer in \cite{dekker1984stability} proved the existence of a fourth-order explicit RK method that can preserve the quadratic invariant For the system. The standard projection method that combines the RK method and an orthogonal projection onto the invariant manifold at each time step is another well-known technique to preserve nonlinear invariants for systems. This method's downside is that it does not preserve the linear invariants that are preserved by the underlying RK methods, making it unfavorable in many applications. Using this projection idea and embedded RK methods, Calvo et al. employed general search directions to advance the solution in time, generalizing the approach in \cite{calvo2006preservation} to any high-order explicit RK methods. They also generalized their methods to conserve several invariants of a system using multiple embedded RK methods. Recently, a modification of these ideas, known as  relaxation \cite{ketcheson2019relaxation,ranocha2020relaxation_1} has been proposed in order to impose dissipation or conservation of general nonlinear functionals while retaining the full accuracy of the original method. This approach was successfully applied to Hamiltonian systems to preserve the Hamiltonians \cite{ranocha2020relaxation} and was further generalized in the context of multistep methods \cite{ranocha2020general}. 
    
    All the applications mentioned above of relaxation methods focus on conserving one invariant for a system. Preserving a single generic invariant requires solving a nonlinear equation for one relaxation parameter at each time step of the method. Our goal in this work is to generalize the idea of relaxation to the system with multiple invariants and see the effects in numerical solutions. The concept of relaxation with multiple invariants uses several lower embedded methods and modified search directions based on those embedded methods. This idea is similar to the approach in \cite{calvo2006preservation}, but the relaxation approach uses one less number of embedded pairs than the approach described by Calvo et al. in \cite{calvo2006preservation}. Conserving $\ell(\geq 1)$ invariants by the relaxation approach needs to solve a nonlinear system for $\ell$ relaxation parameters at each time step. The main contributions of this work are: (a) the generalization of the relaxation approach to conserving several invariants, (b) proof of the existence of relaxation parameters, and (c) the demonstration of the benefits of preserving more than one invariant via several numerical examples. 
    %In section 2, we briefly review relaxation RK methods for one invariant and generalize this approach for several invariants in section 3. The proof of the existence of relaxation parameters is given in section 4. Several numerical experiments are carried out in section 5 to demonstrate how our methodology performs on several test problems. Finally, we close with a conclusion in section 6.
    
	\section{Runge-Kutta Methods and Their Relaxation Versions}
	An $\mathrm{s}$-stage RK method can be presented via its \emph{Butcher tableau}:
    \begin{equation}\label{B_table_RK}
        \renewcommand\arraystretch{1.2}
        \begin{array}
            {c|c}
            \vec{c} & A\\
            \hline
            & \vec{b}^{\,T}
        \end{array}\;, 
    \end{equation}
    where the matrix $A = (a_{ij})\in \Real^{s \times s}$ and vector $\vec{b} \in \Real^{s}$.  We assume 
    \begin{align} \label{c-assumption}
    \vec{c} = A\vec{e},
    \end{align}
    where $\vec{e}$ is the vector of ones in $\Real^{s}$.
    
	For an initial value problem
    \begin{equation}\label{IVP_2}
             \dot{u}(t)  = f\left(t,u(t)\right), \  u(0) = u_{0}; \ u\in \Real^{m}, \ f : \Real\times\Real^m \to \Real^m,
    \end{equation}
    RK methods calculate the numerical solution as
    \begin{subequations}\label{RK_methods}
        \begin{align}
            g_i & = u^n+\Delta t \sum_{j = 1}^{s} a_{ij} f(t_n+c_j \Delta t, g_j), \ i = 1,2, \ldots,s \;, \label{RK_methods_a}\\
            u^{n+1} & = u^{n}+\Delta t \sum_{j = 1}^{s} b_j f(t_n+c_j \Delta t, g_j)\;, \label{RK_methods_b}
        \end{align}
    \end{subequations}
    
    % \begin{align}\label{RK_methods_0}
    %     u^{n+1} & = u^{n}+\Delta t \sum_{j = 1}^{s} b_j f(t_n+c_j \Delta t, g_j),
    % \end{align}
    % where
    % \begin{align}\label{RK_methods_2}
    %     g_i & = u^n+\Delta t \sum_{j = 1}^{s} a_{ij} f(t_n+c_j \Delta t, g_j), \ i = 1,2, \ldots,s \;,
    % \end{align} 
    
    where $\Delta t$ is a time step size, $u^n$ and $u^{n+1}$ are the numerical approximations to the true solution at time $t_n$ and $t_{n+1} = t_n+\Delta t$, respectively. Assume that the system \eqref{IVP_2} has a scalar conserved quantity $G_1:\Real^{m} \to \Real$, i.e., $G_1$ remains constant along each solution. In general, RK methods do not preserve this qualitative behavior discretely. To remedy this one may use a slight modification (known as relaxation) \cite{ketcheson2019relaxation,ranocha2020relaxation_1,ranocha2020relaxation} in which the update
    \begin{align}\label{RRK_methods_1}
        u^{n+1}_{\gamma} & = u^{n}+\gamma \Delta t \sum_{j = 1}^{s} b_j f(t_n+c_j \Delta t, g_j),
    \end{align}
    is used instead of \eqref{RK_methods_b}, where $\gamma \in \Real$ is a scalar that is chosen by imposing the discrete conservation property 
    \begin{align} \label{eq:conservation}
       G_1(u^{n+1}_{\gamma})  =  G_1(u^{n}) \;.
    \end{align}
    The nonlinear algebraic equation \eqref{eq:conservation} must be solved at each time step.  For a $p$th order baseline RK method, it can be shown that there exists a solution satisfying $\gamma = 1+\mathcal{O}(\Delta t^{p-1})$ (under some restrictions) \cite{ketcheson2019relaxation,ranocha2020relaxation_1}. Consequently, the relaxation RK method defined by \eqref{RK_methods_a} and \eqref{RRK_methods_1} has order $p$ when the new updated solution is interpreted as an approximation of the true solution at time $t_n+\gamma \Delta t$. 

\subsection{Embedded Runge-Kutta Sets}

    In the next section we extend the relaxation idea to enforce conservation of multiple invariants.  In order to do so, we require multiple candidate new solutions $u^{n+1}$ that are all of sufficient accuracy.  A convenient and inexpensive way to obtain such solutions utilizes the concept of embedded RK methods.  

    We say a set of RK methods is embedded if all methods in the set share the same coefficient matrix $A$, with different weight vectors $b$.
    Thus the $k$th method in the set has coefficients
    denoted by $(A,b^k)$.  To apply such a set of methods, the stage equations \eqref{RK_methods_a}
    need only be solved once, after which the simple arithmetic updates
     \begin{align}\label{RK_methods_1}
        u^{n+1,k} & = u^{n}+\Delta t \sum_{j = 1}^{s} b_j^k f(t_n+c_j \Delta t, g_j),
    \end{align} 
    can be computed.  No additional evaluations of $f$ or solutions of algebraic equations are required.
    
    Traditional use of embedded methods has focused on pairs, in which one method is designed to have lower order and the difference between the two solutions is used as an estimate of the local error.  Here, in contrast, we will make use of sets consisting of $\ell\ge 2$ methods, and solutions from all methods in the set will be used as part of the numerical solution update.  Ideally, all methods in the set would have the same order of accuracy.  In the numerical examples in this work, we mainly make use of existing methods, and leave the design of RK sets with equal order of accuracy to future work.

    
	\section{Generalization of Relaxation Runge-Kutta Methods for Multiple Invariants}
	So far the relaxation approach has been applied to conserve one quantity of a differential system. We generalize this methodology to conserve multiple nonlinear invariants. Assume now the system of differential equations has $\ell$ smooth invariant  functions $G_1(u)$, $G_2(u)$,...,$G_{\ell}(u)$ defined in a solution space in $\mathbb{R}^m$ and we define
    \begin{align} \label{l-invariants}
        G := (G_1,G_2, \ldots, G_{\ell})^{T}: \mathbb{R}^m \to \mathbb{R}^{{\ell}} \;.
    \end{align}
    The basic idea to conserve $\ell \geq 1$ invariants is to make use $({\ell}-1)$ linearly-independent embedded RK methods each of $(p-1)$th order along with a $p$th order RK method and find a suitable direction in the plane spanned by directions induced by those ${\ell}$ methods so that the invariants are preserved:
    \begin{align} \label{relaxation-equations}
        G_i(u^{n+1}_{\vec{\gamma}}) & = G_i(u^n) & 1 \le i \le \ell.
    \end{align}
    Here the updated solution $u^{n+1}_{\vec{\gamma}}$ is computed using given ${\ell}$ linearly independent embedded RK methods as
    \begin{subequations}\label{modified_Update_rule}
        \begin{align}
            u^{n+1}_{\vec{\gamma}}  & := u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \;, \label{modified_Update_rule_a} \\
            d_{k}^{n} & :=\sum_{j = 1}^{s} b_{j}^{k} f(t_n+c_j \Delta t, g_j), \ \text{for} \ k = 1,2,...,{\ell}\;, \label{increments}
        \end{align}
    \end{subequations}
    where $u^{n+1}=u^{n}+ \Delta t d_{1}^{n}$, $\vec{\gamma} = (\gamma_{1},\gamma_{2},\ldots, \gamma_{{\ell}}) \in \Real^{\ell}$, and stage values $g_i$'s are defined in \eqref{RK_methods_a}. The directions are computed according to given embedded RK methods $(A,\vec{b}^1,\vec{b}^2,\cdots,\vec{b}^{\ell})$
	where, by convention, the first method defined by the vector ${\vec{b}^1} = [b^{1}_{1},b^{1}_{2},\ldots, b^{1}_{s}]^T$ is of order $p$, and the vectors $\vec{b}^j = [b^{j}_{1},b^{j}_{2},\ldots, b^{j}_{s}]^T$ for $j=2,3,\ldots, \ell$ determine the $(\ell-1)$ embedded RK methods each of order $(p-1)$. At each step, we now require to solve a nonlinear system of $\ell$ equations in $\ell$ unknowns $(\gamma_1, \gamma_2,…,\gamma_{\ell})$. The update rule \eqref{modified_Update_rule} here, unlike in  \eqref{RRK_methods_1}, uses $u^{n+1}$ instead of $u^{n}$, which provides better robustness and makes it easier to find relaxation parameters. Notice that this update rule for preserving multiple invariants also applies to a single invariant case. In the case of $\ell = 1$, we only require a $p$th order RK method without any lower order embedded methods. 

	\section{Existence of Relaxation Parameters and Accuracy of the Methods}
    % \begin{theorem}
    %   Suppose the IVP \ref{IVP} has $\ell \geq 1$ smooth conserved quantities defined by the map $G: \mathbb{R}^m \to R^{\ell}$, $G(u) := (G_1(u),G_2(u), \ldots, G_{\ell}(u))^{T}$, and $\left(\nabla G(u^{n+1})\right)^{T} T_n = M(u^n) \Delta t + \mathcal{O}(\Delta t^2)$ holds with non-singular $M(u^n)$, where $T_n = [w_{1}^{n}|\ldots|w_{\ell}^{n}]$  with $w_{k}^{n} = \frac{d_{k}^{n}}{||d_{k}^{n}||}$ for $k=1,2,\ldots, \ell$. Then there exists $\Delta t^{*} > 0$ and a unique set $\left(\gamma_1(u^n,\Delta t), \gamma_2(u^n,\Delta t),\ldots, \gamma_{\ell}(u^n,\Delta t)\right)$ such that the method \ref{modified_Update_rule} defined above preserves $\ell$ invariants $G_i$ for $i=1,2,\ldots, \ell$ with any $\Delta t \in [0,\Delta t^{*}]$, and the method has order $p$.
    % \end{theorem}
    % \begin{proof}
    %     We adapt the proof of \cite[Theorem 4.2]{calvo2006preservation} that relies on the implicit function theorem, to our setting as follows:
    %     \begin{align}
    %         u^{n+1}_{\vec{\gamma}} & = u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \\
    %         u^{n+1}_{\vec{\lambda}} & = u^{n+1} - \sum_{i=1}^{{\ell}} \lambda_{i} w_{i}^{n} \;,
    %     \end{align}
    %     where $w_{i}^{n} = \frac{d_{i}^{n}}{||d_{i}^{n}||}$ and $\gamma_{i} = \frac{-\lambda_{i}}{||\Delta t d_{i}^{n}||}$ for $i=1,2,\ldots, \ell$. Under the condition $\left(\nabla G(u^{n+1})\right)^{T} T_n = M(u^n) \Delta t + \mathcal{O}(\Delta t^2)$ with non-singular $M(u^n)$, theorem 4.2 from \cite{calvo2006preservation} guarantees the existence of a $\Delta t^{*} > 0$ and a unique set $$\left(\lambda_1(u^n,\Delta t), \lambda_2(u^n,\Delta t),\ldots, \lambda_{\ell}(u^n,\Delta t)\right)$$
    %     such that, for any $\Delta t \in [0,\Delta t^{*}]$, the method defined above applied with these set of relaxation parameters, preserves $\ell$ invariants and has order $p$. Applying the relation between the vectors $\vec{\gamma}$ and $\vec{\lambda}$, it follows the final results.
    % \end{proof}
    \begin{lemma}
        Suppose that the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants} and a set of embedded Runge-Kutta methods $(A,b^1,\dots,b^\ell)$, each of order $p\geq 2$, $u^n \in \Real^m$, and $\Delta t \ge 0$ be given. Let $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$  with $d_{k}^{n}$ defined in \eqref{increments}. If 
        $$\nabla G(u^{n+1}) \cdot D_n = B(u^n)\Delta t+\O(\Delta t^2)$$
        holds with non-singular $B(u^n)$ and $B^{-1}=\O(1)$, then there exists $\Delta t^{*} > 0$ such that for every $\Delta t \in [0,\Delta t^{*}]$ there is a unique vector $\vec{\gamma}$ 
        such that equations \eqref{relaxation-equations}-\eqref{modified_Update_rule} are satisfied and 
        $$\gamma_{i} = \O(\Delta t^{p-1}), \ \text{for } \ i = 1,2,\cdots, \ell.$$
    \end{lemma}
    \begin{proof}
        Consider the real function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
        \begin{align}\label{Lemma_eq1}
            g(\Delta t, \vec{\gamma}) :=      
           \frac{G\left(u^{n+1}_{\vec{\gamma}}\right)- G(u^{n})}{\Delta t^2}, & \ \text{for} \ \Delta t \neq 0 \;, 
        \end{align}
        where $u^{n+1}_{\vec{\gamma}}$ is defined in \eqref{modified_Update_rule_a}. Applying the Taylor's theorem with $h_n  := \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}$ we obtain 
        \begin{align}\label{Lemma1_eq2}
             G(u^{n+1}_{\vec{\gamma}})=G\left(u^{n+1}+ \Delta t h_n\right) = G(u^{n+1}) + \Delta t \nabla G(u^{n+1}) \cdot h_{n} + \Delta t^2 \frac{D^2g(u^{n+1})}{2!}(h_{n},h_{n}) +\O(\Delta t^3).
        \end{align}
        Also, note that the numerical solutions of an RK method of order $p$ satisfy 
        \begin{align*}
            G_i(u^{n+1})- G_i(u^{n}) & = G_i\left(u(t_{n+1})+\O(\Delta t^{p+1})\right) - G_i\left(u(t_{n})+\O(\Delta t^{p+1})\right) \;, \\
            & = G_i\left(u(t_{n+1})\right) - G_i\left(u(t_{n})\right) +\O(\Delta t^{p+1})\;, \\
            & = \int_{t_n}^{t_n+\Delta t}\frac{\textrm{d}}{\textrm{dt}}G_i\left(u(t)\right)dt +\O(\Delta t^{p+1})\;, \\
            & = \O(\Delta t^{p+1})\;, \ \text{since} \ \frac{\textrm{d}}{\textrm{dt}}G_i\left(u\right) = 0, \ \text{by assumption.}
        \end{align*}
        This holds for $i=1,2,\cdots, \ell$ and hence 
        \begin{align}\label{accuracy_diff_G}
            G(u^{n+1})- G(u^{n}) = \O(\Delta t^{p+1}) \;.
        \end{align}
        Using the assumption, \eqref{Lemma1_eq2}, and \eqref{accuracy_diff_G} in \eqref{Lemma_eq1} we write
        \begin{align*}\label{Lemma1_eq3}
             g(\Delta t, \vec{\gamma}) & = \Delta t^{-2} \left[ G\left(u^{n+1}+ \Delta t h_n\right) - G(u^{n})\right] \;, \\
             & = \Delta t^{-2} \left[ G(u^{n+1}) + \Delta t \nabla G(u^{n+1}) \cdot h_{n} + \Delta t^2 \frac{D^2g(u^{n+1})}{2!}(h_{n},h_{n}) +\O(\Delta t^3) - G(u^{n})\right] \;, \\
             & = \frac{G(u^{n+1})- G(u^{n})}{\Delta t^2} + \Delta t^{-1} \nabla G(u^{n+1}) \cdot D_{n} \vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n}) +\O(\Delta t) \;, \\
             & = \O(\Delta t^{p-1}) + \left(B(u^n)+\O(\Delta t)\right)\vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})+\O(\Delta t)\;, \\
             & = \left(B(u^n)+\O(\Delta t)\right)\vec{\gamma}+\frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})+\O(\Delta t), \ \text{since} \ p \geq 2 \;.
        \end{align*}
        Thus we define, 
        \begin{align}
            g(0,\vec{\gamma}):=\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = B(u^n)\vec{\gamma}+\left. \frac{D^2g(u^{n+1})}{2!} (h_{n},h_{n})\right|_{\Delta t = 0}\;,
        \end{align}
        and then $g(\Delta t,\vec{\gamma})$ is continuous for all $\Delta t \geq 0$. Notice that $g(0,\vec{0}) = 0$. Furthermore, the function is differentiable with respect to $\Vec{\gamma}$ and the Jacobian is given by
        $$J_{g,\vec{\gamma}}(0,\vec{0}) = B(u^n).$$
        Since $B(u^n)$ is non-singular by assumption, the implicit function theorem guarantees the existence of a $\Delta t^{*} > 0$ and a unique function $$\vec{\gamma}(\Delta t) = \left(\gamma_1(\Delta t), \gamma_2(\Delta t),\ldots, \gamma_{\ell}(\Delta t)\right)$$
        such that, for any $\Delta t \in [0,\Delta t^{*}]$ we have $\vec{\gamma}(0) = \vec{0}$ and $g(\Delta t,\vec{\gamma}(\Delta t)) = 0$. Hence it follows from \eqref{Lemma_eq1} that the method defined in \eqref{modified_Update_rule} applied with these set of relaxation parameters will satisfy the $\ell$-invariant equations given by \eqref{relaxation-equations} for the system. 
        
        To know the accuracy of $\vec{\gamma}$ consider the expansion
        \begin{align}\label{Lemma1_eq4}
            g(\Delta t,\vec{\gamma}) = g(\Delta t,\vec{0}) + J_{g,\vec{\gamma}}(\Delta t,\vec{0}) \cdot \vec{\gamma} + \mathcal{O}(||\vec{\gamma}||^2) 
        \end{align}
        with 
        \begin{align}\label{Lemma1_eq5}
            g(\Delta t,\vec{0}) = \frac{G(u^{n+1})- G(u^{n})}{\Delta t^2} = \mathcal{O}(\Delta t^{p-1}), \ \text{by} \ \eqref{accuracy_diff_G} \;,
        \end{align} 
        and 
        \begin{align}\label{Lemma1_eq6}
            J_{g,\vec{\gamma}}(\Delta t,\vec{0}) = J_{g,\vec{\gamma}}(0,\vec{0}) + \mathcal{O}(\Delta t) = B(u^n) +\mathcal{O}(\Delta t) \;. 
        \end{align}
        Using \eqref{Lemma1_eq4}, \eqref{Lemma1_eq5}, \eqref{Lemma1_eq6}, and the assumption $B^{-1}=\O(1)$ we conclude that each component of the vector $\vec{\gamma}$ is $\mathcal{O}(\Delta t^{p-1})$.     
    \end{proof}

    \begin{theorem}
        Let the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants} and $(A,b^1,\dots,b^\ell)$ be the coefficients of a set of $\ell$ embedded Runge-Kutta methods each of order $p\geq 2$. Consider the generealized relaxation method defined by \eqref{relaxation-equations}-\eqref{modified_Update_rule} and assume $\vec{\gamma} = \O(\Delta t^{p-1})$, then:
        \begin{enumerate}
            \item If the solution $u^{n+1}_{\vec{\gamma}}$ is interpreted as an approximation to $u(t_n+\Delta t)$, the method has order $p-1$.
            \item The generalized relaxation method interpreting $u^{n+1}_{\vec{\gamma}}$ as an approximation to $u(t^{n+1}_{\vec{\gamma}})$ has order $p$, where $t^{n+1}_{\vec{\gamma}}=t_n+\left(1+\sum \gamma_{i} \right)\Delta t$.
        \end{enumerate}
    \end{theorem}
    \begin{proof}
        Let $\mathbf{f} := [f(t_n+c_1 \Delta t, g_1)|f(t_n+c_2 \Delta t, g_2)| \ldots| f(t_n+c_s \Delta t, g_s)]$ be the matrix of stage vectors, $\mu_1 := 1+\gamma_1$, and $\mu_i := \gamma_i$ for $i = 2,3,\cdots, \ell$. Then the modified update rule \eqref{modified_Update_rule_a} can be rewritten as
        \begin{equation}
            \begin{aligned}
                u^{n+1}_{\vec{\gamma}} & = u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \;, \\
                & = u^{n}+\Delta  t \sum_{i=1}^{{\ell}} \mu_{i} \mathbf{f} \vec{b}^{i}, \ \text{using} \ \eqref{increments} \;, \\
                & = u^{n}+\Delta  t \mathbf{f}  \sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\;. \\
            \end{aligned}
        \end{equation}
        So we can view the update rule of the generalized relaxation method as applying the following RK method to the system:
        \begin{equation}\label{diff_formulation_GRRRK_mthd}
            \renewcommand\arraystretch{1.2}
            \begin{array}
            {c|c}
            \vec{c} & A\\
            \hline
            & \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{\,T}
            \end{array}\;.
        \end{equation}
        Following the proof of \cite[Theorem 2.7]{ketcheson2019relaxation}, we use an equivalent set of order conditions \cite{albrecht1996runge}
        \begin{subequations}
            \begin{align}
                \vec{b}^{\,T}\vec{c}^{\, k-1} - 1/k & = 0, & 1 \le k \le p, \\
                \vec{b}^{\,T} v & = 0 & \forall v \in V_{p},
            \end{align}
        \end{subequations}
        for an RK method \eqref{B_table_RK} to have an order $p$, where $V_{p}$ is a set of vectors depending only on the coefficients of $A$. 
        
        If $u^{n+1}_{\vec{\gamma}} \approx u(t_n+\Delta t)$, in view of \eqref{diff_formulation_GRRRK_mthd}, the order conditions for the generalized relaxation RK methods can be obtained by replacing $\vec{b}^{\,T}$ with $\left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}$:
        \begin{subequations}
            \begin{align}
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - 1/k & = 0, & 1 \le k \le p, \label{IDT_OC_a} \\
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T} v & = 0 & \forall v \in V_{p}, \label{IDT_OC_b}
            \end{align}
        \end{subequations}
        Since each of the embedded methods has order $p$, it follows that for all $i$, $(\vec{b}^{i})^{\,T} v = 0, \ \forall \ v \in V_{p}$ and hence \eqref{IDT_OC_b} is satisfied. On the other hand, the accuracy of $\mu_i$'s and the order of embedded methods implies that the left hand side of equation \eqref{IDT_OC_a} is $\O(\Delta t^{p-1})$. This quantity gets multiplied by $\O(\Delta t^{k})$ in the error expansion producing the leading order term as $\O(\Delta t^{p})$; hence the method has order $p-1$.
        
        When we interpret the solution $u^{n+1}_{\vec{\gamma}}$ as an approximation to $u(t^{n+1}_{\vec{\gamma}}) = u(t_n+\left(\sum \mu_{i} \right)\Delta t)$, we view the numerical solution $u^{n+1}_{\vec{\gamma}}$ as an interpolant of the RK method's \eqref{diff_formulation_GRRRK_mthd} solution, evaluated at $\left(\sum \mu_{i} \right)\Delta t$. Then the set of order conditions for this interpolated solution becomes
        \begin{subequations}
            \begin{align}
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - \frac{\left(\sum \mu_{i} \right)^k}{k} & = 0, & 1 \le k \le p, \label{GRRRK_OC_a} \\
                \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T} v & = 0 & \forall v \in V_{p}. \label{GRRRK_OC_b}
            \end{align}
        \end{subequations}
        Notice that equation \eqref{GRRRK_OC_b} is the same as condition \eqref{IDT_OC_b}, so the order conditions in \eqref{GRRRK_OC_b} are satisfied. It is easy to see that the equation in \eqref{GRRRK_OC_a} for $k=1$ is also exactly satisfied. For $k \geq 2$, we write 
        \begin{align}
            \left(\sum_{i=1}^{{\ell}} \mu_{i} \vec{b}^{i}\right)^{T}\vec{c}^{\, k-1} - \frac{\left(\sum \mu_{i} \right)^k}{k} & =  \sum_{i=1}^{{\ell}} \frac{\mu_{i}}{k}  - \frac{\left(\sum \mu_{i} \right)^k}{k} \;, \\
            & = \frac{\sum \mu_{i}}{k} \left(1-\left(\sum \mu_{i}\right)^{k-1}\right)\;, \\
            & = \frac{\sum \mu_{i}}{k} \left(1-\left(1+\O(\Delta t^{(p-1)(k-1)})\right)\right)\;, \\
            & = \O\left(\Delta t^{(p-1)(k-1)}\right) \;.
        \end{align}
        Each of these residuals gets multiplied by $\O(\Delta t^k)$ in the error expansion, and the error term becomes $\O\left(\Delta t^{(k-1)p+1}\right)$. This makes the leading order error term $\O\left(\Delta t^{p+1}\right)$ for $k \ge 2$; hence, the method has order $p$.
    \end{proof}
    
    % \begin{theorem}
    %     Let $u^n \in \Real^m$, a set of embedded Runge-Kutta methods $(A,b^1,\dots,b^\ell)$, and $\Delta t \ge 0$ be given.  Let $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$  with $d_{k}^{n}$ defined in \eqref{increments}.
    %    Suppose that the IVP \eqref{IVP_2} has $\ell \geq 1$ smooth conserved quantities \eqref{l-invariants}
    %    %defined by the map $G: \mathbb{R}^m \to \mathbb{R}^{\ell}$, $G(u) := (G_1(u),G_2(u), \ldots, G_{\ell}(u))^{T}$, 
    %    and that 
    %    $$\left(\nabla G(u^{n})\right)^{T} \cdot D_n = M(u^n)$$
    %     holds with non-singular $M(u^n)$.  Then there exists $\Delta t^{*} > 0$ such that for every $\Delta t \in [0,\Delta t^{*}]$ there is
    %      a unique vector $\vec{\gamma}$ %$\left(\gamma_1(u^n,\Delta t), \gamma_2(u^n,\Delta t),\ldots, \gamma_{\ell}(u^n,\Delta t)\right)$ 
    %     such that equations \eqref{relaxation-equations}-\eqref{increments} are satisfied.

    %     Let $p$ denote the minimum order of accuracy of the Runge-Kutta methods in the set.  Then
    %     $$
    %         u^{n+1}_{\vec{\gamma}} = u\left(t_n+\left(1+\sum_i \gamma_i\right) \Delta t\right) + {\mathcal O}(\Delta t^{p+1}).
    %         $$
    % \end{theorem}
    % \begin{proof}
    %     % Consider the function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
    %     % \begin{align}\label{Existence_proof_eq1}
    %     %     g(\Delta t, \vec{\gamma}) :=
    %     %     \begin{cases}
    %     %                  \frac{G\left(u^{n+1}_{\vec{\gamma}}\right)- G(u^{n})}{\Delta t} & \text{if} \ \Delta t \neq 0 \\
    %     %                  C^{*} &  \text{if} \ \Delta t = 0 \;,
    %     %     \end{cases}
    %     % \end{align}
    %     % where $C^{*}$ is defined as $C^{*} := \displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = \nabla G(u^{n}) \cdot \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right)$.
        
    %     % {\color{blue} With $h_n  := \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right) $, we write
    %     % \begin{align*}
    %     %     g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^n+ \Delta t h_n\right) - G(u^{n})\right] \\
    %     %     & = \frac{1}{\Delta t} \left[ G(u^n) + \Delta t \nabla G(u^n) \cdot  h_n + \mathcal{O}(\Delta t^2)  - G(u^{n})\right].
    %     % \end{align*}
    %     % Hence $\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} =\nabla G(u^n) \cdot  h_n = \nabla G(u^{n}) \cdot \left( d_{1}^{n} + \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \right)$.
    %     % }
        
    %     % Since $G$ is a continuously differentiable function, using the mean value theorem we obtain 
    %     % \begin{align*}
    %     %      G\left(u^n+ \Delta t h_n\right) - G(u^{n}) = \left(\int_{0}^{1} \nabla G(u^n + \theta \Delta t h_n ) \ d\theta \right) \cdot \Delta t h_n.
    %     % \end{align*}
    %     % Then for $\Delta t \neq 0$ we have 
    %     % \begin{align}\label{Existence_proof_eq2}
    %     %      g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^n+ \Delta t h_n\right) - G(u^{n})\right] = \left(\int_{0}^{1} \nabla G(u^n + \theta \Delta t  h_n ) \ d\theta \right) \cdot h_n.
    %     % \end{align}
        
    %     Consider the function $g : \mathbb{R}\times\mathbb{R}^{\ell} \to \mathbb{R}^{\ell}$ defined by 
    %     \begin{align}\label{Existence_proof_eq1}
    %         g(\Delta t, \vec{\gamma}) :=      
    %              \frac{G\left(u^{n+1}_{\vec{\gamma}}\right)- G(u^{n})}{\Delta t}, & \ \text{for} \ \Delta t \neq 0 \;,    
    %     \end{align}
        
    %     where $g(0,\vec{\gamma})$ is given by the corresponding limit 
    %     \begin{align}
    %         g(0, \vec{\gamma}):=\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} =\nabla G(u^{n+1}) \cdot  h_n + \mathcal{O}(\Delta t)= \nabla G(u^{n}) \cdot h_n  \;,
    %     \end{align}
    %     where $h_n  := \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n}$.
    %     Since $G$ is a continuously differentiable function, using the mean value theorem we obtain 
    %     \begin{align*}
    %          G\left(u^{n+1}+ \Delta t h_n\right) = G(u^{n+1}) + \left(\int_{0}^{1} \nabla G(u^{n+1} + \theta \Delta t h_n ) \ d\theta \right) \cdot \Delta t h_n.
    %     \end{align*}
    %     Then for $\Delta t \neq 0$ we have 
    %     \begin{align}\label{Existence_proof_eq2}
    %          g(\Delta t, \vec{\gamma}) & = \frac{1}{\Delta t} \left[ G\left(u^{n+1}+ \Delta t h_n\right) - G(u^{n})\right] \\
    %          & = \frac{G(u^{n+1})- G(u^{n})}{\Delta t}+\left(\int_{0}^{1} \nabla G(u^{n+1} + \theta \Delta t  h_n ) \ d\theta \right) \cdot h_n.
    %     \end{align}
        
        
    %     Using \eqref{Existence_proof_eq2}, we conclude that $\displaystyle{\lim_{\Delta t \to 0} g(\Delta t, \vec{\gamma})} = \nabla G(u^{n}) \cdot h_n$, and hence $g$ is continuous function at $\Delta t = 0$. Taking into account the smoothness of $G$, it is easy to see that $g$ is differentiable with respect to $\vec{\gamma}$ and the derivative is also a continuous in a neighbourhood of the origin. Observe that $g(0,\vec{0}) = \vec{0}$ and the Jacobian is given by
    %     \begin{align}
    %         J_{g,\vec{\gamma}}(0,\vec{0}) = (\nabla G(u^n))^T \cdot D_n = M(u^n) \;,
    %     \end{align}
    %     where $D_n = [d_{1}^{n}|\ldots|d_{\ell}^{n}]$. 
    %     {\color{blue}
    %     \begin{align*}
    %            J_{g,\vec{\gamma}}(\Delta t,\vec{\gamma}) = & \frac{1}{\Delta t}
    %             \begin{bmatrix}
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{1} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n}\\
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{2} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n}\\
    %                 \vdots & \\
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{1}^{n} & 
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{2}^{n} &
    %                 \ldots &
    %                 \ldots &
    %                 \nabla G_{\ell} (u^{n+1}_{\vec{\gamma}}) \cdot \Delta t d_{\ell}^{n} \;,
    %             \end{bmatrix} \\
    %             & = (\nabla G(u^{n+1}_{\vec{\gamma}}))^T \cdot D_n \;.
    %     \end{align*}
    %     }
    %     Since $M(u^n)$ is non-singular by assumption, the implicit function theorem guarantees the existence of a $\Delta t^{*} > 0$ and a unique set $$\left(\gamma_1(u^n,\Delta t), \gamma_2(u^n,\Delta t),\ldots, \gamma_{\ell}(u^n,\Delta t)\right)$$
    %     such that, for any $\Delta t \in [0,\Delta t^{*}]$ we have $g(\Delta t,\vec{\gamma}) = 0$. Hence the method defined above applied with these set of relaxation parameters, will preserve $\ell$ invariants for the system. 
        
    %     Consider the expansion
    %     \begin{align}\label{Existence_proof_eq3}
    %         g(\Delta t,\vec{\gamma}) = g(\Delta t,\vec{0}) + J_{g,\vec{\gamma}}(\Delta t,\vec{0}) \cdot \vec{\gamma} + \mathcal{O}(||\vec{\gamma}||^2) 
    %     \end{align}
    %     with \begin{align}\label{Existence_proof_eq4}
    %         g(\Delta t,\vec{0}) = \frac{G(u^{n+1})- G(u^{n})}{\Delta t} = \mathcal{O}(\Delta t^p) \;,
    %     \end{align} 
    %     and 
    %     \begin{align}\label{Existence_proof_eq5}
    %         J_{g,\vec{\gamma}}(\Delta t,\vec{0}) = J_{g,\vec{\gamma}}(0,\vec{0}) + \mathcal{O}(\Delta t) = M(u^n) +\mathcal{O}(\Delta t) \;. 
    %     \end{align}
    %     Using \eqref{Existence_proof_eq3}, \eqref{Existence_proof_eq4}, and \eqref{Existence_proof_eq5} we conclude that each component of the vector $\vec{\gamma}$ is $\mathcal{O}(\Delta t^p)$.
    %     The accuracy of the $p$th order baseline method and each $\gamma_{i}$ being $\mathcal{O}(\Delta t^p)$ imply that 
    %     \begin{equation}\label{Existence_proof_eq6}
    %         \begin{aligned}
    %         u^{n+1}_{\vec{\gamma}} & = u^{n+1}+\Delta  t \sum_{i=1}^{{\ell}} \gamma_{i} d_{i}^{n} \\
    %         & = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1})\;.
    %         \end{aligned}
    %     \end{equation}

    %     On the other hand when the numerical solution is considered as an approximation at $t^{n+1}_{\vec{\gamma}} = t^{n+1}+\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}$, using Taylor expansion we obtain 
    %     \begin{align}\label{Existence_proof_eq7}
    %         u(t^{n+1}_{\vec{\gamma}}) = u(t_{n+1}) + \dot{u}(t_{n+1})\left(\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}\right) + \mathcal{O}\left(\left(\Delta t \sum_{i=1}^{{\ell}} \gamma_{i}\right)^2\right) = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1}) \;.
    %     \end{align}
    %     The result $u^{n+1}_{\vec{\gamma}} - u(t^{n+1}_{\vec{\gamma}}) = \mathcal{O}(\Delta t^{p+1}) $ follows from \eqref{Existence_proof_eq6} and \eqref{Existence_proof_eq7}, and hence the relaxation method has order $p$.

        
    %     % The accuracy of the $p$th order baseline method and the $(p-1)$th order embebdded method imply that 
    %     % \begin{align}
    %     %     u^{n+1} = u(t_{n+1}) + \mathcal{O}(\Delta t^{p+1}) \ \text{and} \  u^{n+1,i} = u(t_{n+1}) + \mathcal{O}(\Delta t^{p}) \;,
    %     % \end{align}
    %     % where $u^{n+1}=u^{n}+\Delta t d_{1}^{n}$ and $u^{n+1,i} = u^{n}+\Delta t d_{i}^{n}$ are the approximate solutions by the baseline method and the $i$th embedded method, respectively, at time $t_{n+1}$, for $i=2,\ldots, \ell$. Using these equations we obtain
    %     % \begin{align}
    %     %     \Delta t d_{1}^{n} = u^{n+1}-u^{n} =   u(t_{n+1}) - u(t_{n}) + \mathcal{O}(\Delta t^{p+1}) = \mathcal{O}(\Delta t^{}) 
    %     % \end{align}
    % \end{proof}


	\section{Numerical Examples}
    To demonstrate that the idea of relaxation with multiple invariants works in general, we use several Runge-Kutta methods, apply them to different numerical examples below, and present the results of our numerical experiments. The following numerical schemes with embedded methods are used in the numerical experiments.
    \begin{itemize}
        \item SSPRK(2,2): Two-stages, second-order SSP method with a first-order embedded method.
        \item SSPRK(3,3): Three-stages, third-order SSP method with second-order embedded methods.
        \item Heun(3,3): Three-stages, third-order Heun's method with a second-order embedded method.
        %\item SSPRK(10,4): Ten-stages, fourth-order SSP method with a third-order embedded method.
        \item RK(4,4): Classical four-stages, fourth-order method with a second-order embedded method.
        \item Fehlberg(6,4): Six-stages, fourth-order Fehlberg's method with third-order embedded methods.
        \item DP(7,5): Seven-stages, fifth-order method with fourth-order embedded methods.
        \item ARK3(2)4L[2]SA: Four-stages, third-order additive Runge-Kutta (ARK) method with a second-order embedded ARK method.
        \item ARK4(3)6L[2]SA: Six-stages, fourth-order ARK method with a third-order embedded ARK method.
    \end{itemize}
    The coefficients of two ARK methods, ARK3(2)4L[2]SA and ARK4(3)6L[2]SA, with their embedded pairs, are taken from \cite[Appendix C]{kennedy2003additive}.  The coefficients of the other methods with their lower-order embedded pairs are provided in appendix ~\ref{app:butcherTableau}.
    \subsection{Euler Equations}
    Consider the system of Euler equations that describes the motion of a free rigid body with its center of mass at the origin, in terms of its angular momenta:
    \begin{subequations}\label{Eq:Euler_equations}
        \begin{align}
            &\dot{u}_{1}=(\alpha - \beta)u_2u_3 \\
            &\dot{u}_{2}=(1-\alpha)u_3u_1 \\
            &\dot{u}_{3}=(\beta-1)u_1u_2\;,
        \end{align}
    \end{subequations}
    with $\left(u_1(0),u_2(0),u_3(0)\right)^T = (0,1,1)^T$, $\alpha = 1 + \frac{1}{\sqrt{1.51}}$, and $\beta = 1 - \frac{0.51}{\sqrt{1.51}}$. The exact solution is
    \begin{align}
        \left(u_1(t),u_2(t),u_3(t)\right)^T = \left(\sqrt{1.51} \  \textrm{sn}(t,0.51),\textrm{cn}(t,0.51),\textrm{dn}(t,0.51)\right)^T \;,
    \end{align}
    where $\textrm{sn},\ \textrm{cn},\ \text{and}, \ \textrm{dn}$ are the elliptic Jacobi functions. This problem has two quadratic conserved quantities:
    \begin{subequations}\label{Eq:Euler_invariantas}
       \begin{align}
            & G_1(u_{1},u_{2},u_{3}) = u_{1}^{2}+ u_{2}^{2}+u_{3}^{2} \;, \\
            & G_2(u_{1},u_{2},u_{3}) = u_{1}^{2}+ \beta u_{2}^{2}+\alpha u_{3}^{2} \;.
        \end{align}
    \end{subequations}
    Here $G_{2}$ is the kinetic energy of the body. First, we present the convergence results obtained with different RK and relaxation methods to confirm that relaxation with multiple invariants also produces the desired order of convergence. Using four different RK schemes (second order scheme of Shu \& Osher \cite{shu1988efficient}, third order Heun's method \cite{heun1900neue}, classical fourth order RK method, and Fifth order method of Prince \& Dormand \cite{prince1981high}) and their relaxation versions, we solve the system to a final time of $5$ and report the convergence results in Figure ~\ref{fig:EE_Error_Convergence}.
    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Baseline_Mthds_ErrorConv_tf5.eps}
         \caption{Baseline methods.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Relaxation_Mthds_ErrorConv_tf5.eps}
         \caption{Relaxation methods with multiple invariants.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Convergence of numerical solution by different RK methods and relaxation methods for the Euler's equations.}
    	\label{fig:EE_Error_Convergence}
    \end{figure}

    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Heuns3p3_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{Third order Heun's method, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Fehlbergs6p4_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{Fourth order method of Fehlberg, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_DP5s7p5_InvariantVsTime_dt1e-01_tf1000.eps}
         \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Invariant errors with different methods for Euler's equations. (\Romannum{1}) $G_{1}(t)-G_{1}(0)$: error in the first quadratic invariant over time $t$, (\Romannum{2}) $G_{2}(t)-G_{2}(0)$: error in kinetic energy over time $t$.}
    	\label{fig:EE_Evolution_conserved_quantities}
    \end{figure}
    
    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Heuns3p3_ErrorVsTime_dt1e-01_tf1000.eps}
         \caption{Third order Heun's method, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_Fehlbergs6p4_ErrorVsTime_dt1e-01_tf1000.eps}
         \caption{Fourth order method of Fehlberg, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/EE/EE_DP5s7p5_ErrorVsTime_dt1e-01_tf1000.eps}
          \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time by different methods for Euler's Equations.}
    	\label{fig:EE_error_growth}
    \end{figure}
    Next, we study the error in invariants and the error growth over time by various methods. We integrate the problem with three explicit RK methods and their relaxation versions, third order method of Heun \cite{heun1900neue}, fourth order method of Fehlberg \cite[Table \Romannum{3}]{fehlberg1969low}, and fifth order method of Prince \& Dormand \cite{prince1981high}, with $\Delta t = 0.1$ for all the methods. Figure ~\ref{fig:EE_Evolution_conserved_quantities} plots the error in conserved quantities, confirming that all the relaxation methods preserve both invariants. The error growth by all the methods is plotted in Figure ~\ref{fig:EE_error_growth}, which shows a linear error growth when the two invariants are preserved by the relaxation methods. In contrast, the baseline methods produce errors that increase quadratically.
    %\abhi{The error convergence plots for the odd order methods are not clean. This probably has something to do with the superconvergence, but I am not sure because we use lower-order embedded methods here.}
    
    \subsection{Bi-Hamitonian 3D Lotka-Volterra Systems}
    Next, we consider an ecological predator-prey model of the Lotka-Volterra systems in $3$D, whose equations are given as
    \begin{subequations}\label{Eq:3D_LVS}
        \begin{align}
            &\dot{u}_{1}=u_{1}\left(c u_{2}+u_{3}+\lambda\right) \\
            &\dot{u}_{2}=u_{2}\left(u_{1}+a u_{3}+\mu\right) \\
            &\dot{u}_{3}=u_{3}\left(b u_{1}+u_{2}+\nu\right) \;,
        \end{align}
    \end{subequations}
    where $\lambda, \mu, \nu >0$, $abc=-1$ and $\nu = \mu b - \lambda ab$. We study this problem on the interval $[0,400]$ with parameters $(a,b,c,\lambda,\mu,\nu) = (-1,-1,-1,0,1,-1)$ and the initial condition is taken as $\left(u_1(0),u_2(0),u_3(0)\right)^T = (1,1.9,0.5)^T$. This system has periodic solutions and possesses two nonlinear conserved quantities, known as Casimirs of some skew-symmetric Poisson matrices \cite{ionescu2015geometrical,uzunca2019preservation}:
        \begin{subequations} \label{Eq:3D_LVS_invariants}
            \begin{align}
            & H_1 = ab \ln{u_1} - b \ln{u_2} + \ln{u_3} \;, \\
            & H_2 = ab u_1 + u_2 - a u_3 + \nu \ln{u_2} - \mu \ln{u_3}.
        \end{align}
    \end{subequations}
    
    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Heuns3p3_InvariantVsTime_dt4e-02_tf400.eps}
         \caption{Third order Heun's method, $\Delta t = 0.04$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_RKs4p4_InvariantVsTime_dt1e-01_tf400.eps}
         \caption{Classical fourth order RK method , $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Fehlbergs6p4_InvariantVsTime_dt1e-01_tf400.eps}
         \caption{Fifth order method of Fehlberg, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Invariant errors with different methods for a bi-Hamiltonian $3$D Lotka-Volterra system. (\Romannum{1}) $H_{1}(t)-H_{1}(0)$: error in the first nonlinear invariant over time $t$, (\Romannum{2}) $H_{2}(t)-H_{2}(0)$: error in the second nonlinear invariant over time $t$.}
    	\label{fig:3DLVS_Evolution_conserved_quantities}
    \end{figure}
    We apply third order Heun's method \cite{heun1900neue} with $\Delta t = 0.04$, classical fourth order RK method with $\Delta t = 0.1$, and Fifth order method of Prince \& Dormand \cite{prince1981high}) with $\Delta t = 0.1$ to solve the system with and without relaxation, and obtain numerical solutions. Our observation is that all baseline and relaxation methods preserve the periodicity of the solution. The errors in invariants are shown in Figure ~\ref{fig:3DLVS_Evolution_conserved_quantities}, and we can see that all the relaxation methods preserve the nonlinear invariants for the system over a long time. 
    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Heuns3p3_ErrorVsTime_dt4e-02_tf400.eps}
         \caption{Third order Heun's method, $\Delta t = 0.04$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_RKs4p4_ErrorVsTime_dt1e-01_tf400.eps}
         \caption{Classical fourth order RK method , $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/3DLVS/bi_H_LVS_Fehlbergs6p4_ErrorVsTime_dt1e-01_tf400.eps}
          \caption{Fifth order method of Fehlberg, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth over time by different methods a bi-Hamiltonian $3$D Lotka-Volterra system.}
    	\label{fig:3DLVS_error_growth}
    \end{figure}
    As the closed form of the analytical solution of this system is not known, we use a proxy of the exact solution by using the dense output of the Python "dopri5" method with minimal values for the relative and absolute tolerances. We measure the error in the maximum norm and present the error growth behavior over a long time by all the methods in Figure ~\ref{fig:3DLVS_error_growth}. The invariant-preserving relaxation methods show asymptotic linear error growth and eventually win in solution accuracy over the quadratically increasing errors by the corresponding baseline methods. 
    
    \subsection{Kepler's Problem}
    \subsubsection{The Kepler's Two-Body Problem with Three Invariants}
    So far, all the numerical examples considered above have two conserved quantities for the corresponding system. We now study Kepler's Two-Body problem with three invariants to demonstrate that the relaxation process can conserve more than two invariants for a system. With one of the two bodies fixed at the center of the $2$D plane, the motion of the other body with position $q = (q_{1},q_{2})$ and momentum $p = (p_{1},p_{2})$ is given by the following system of first order differential equations
    \begin{subequations}\label{Eq:Kepler_two_body_problem}
        \begin{align}
            \dot{q_{1}} & = p_{1} \\
            \dot{q_{2}} & = p_{2} \\
            \dot{p_{1}} & = -\frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} \\
            \dot{p_{2}} & =-\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} \;.
        \end{align}
    \end{subequations}
    Three conserved quantities for Kepler's Two-Body system that we consider for our numerical studies are
    \begin{subequations} \label{Eq:Kepler_invariants}
        \begin{align}
            H(q,p) & = \frac{1}{2}\left(p_{1}^2+p_{2}^2\right)-\frac{1}{\sqrt{q_{1}^2+q_{2}^2}} \ (\text{Hamiltonian}) \;, \\
        	L(q,p) & = q_{1}p_{2}-q_{2}p_{1}\ (\text{angular momentum}) \;, \\
        	A(q,p) & = \textrm{$L_2$ norm of Laplace–Runge–Lenz vector} \;,
        \end{align}
    \end{subequations}
   where in the last invariant, the well-known Laplace–Runge–Lenz vector function \cite[Page 26]{haier2006geometric} is defined as 
  \begin{align}
        \begin{bmatrix}
        p_{1} \\
        p_{2} \\
        0
        \end{bmatrix} \times \begin{bmatrix}
        0 \\
        0 \\
        q_{1} p_{2}-q_{2} p_{1}
        \end{bmatrix}-\frac{1}{\sqrt{q_{1}^{2}+q_{2}^{2}}} \begin{bmatrix}
        q_{1} \\
        q_{2} \\
        0
        \end{bmatrix}\;.
   \end{align}
    We consider the Two-Body problem with an initial condition $ \left(q_{1}(0),q_{2}(0),p_{1}(0),p_{2}(0)\right)^{T}=\left(1-e,0,0,\sqrt{\frac{1+e}{1-e}}\right)^{T}$ with $e=0.5$, and study the conservation of invariants in \eqref{Eq:Kepler_invariants} and the global error by different RK methods and their relaxation versions. Three explicit RK methods, third order method of Shu \& Osher \cite{shu1988efficient} with $\Delta t = 0.005$, fourth order method of Fehlberg \cite[Table \Romannum{3}]{fehlberg1969low}, with $\Delta t = 0.05$, and fifth order method of Prince \& Dormand \cite{prince1981high} with $\Delta t = 0.1$ are used as baseline methods to solve the problem.
   \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_SSPRKs3p3_InvariantVsTime_dt5e-03_tf200.eps}
         \caption{Third order method of Shu \& Osher, $\Delta t = 0.005$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_Fehlbergs6p4_InvariantVsTime_dt5e-02_tf200.eps}
         \caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_DP5s7p5_InvariantVsTime_dt1e-01_tf200.eps}
         \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Errors in conserved quantities \eqref{Eq:Kepler_invariants} by different methods for Kepler's Two-Body problem. (\Romannum{1}) $H_{t}-H_{0}$: error in Hamiltonian over time $t$, (\Romannum{2}) $L_{t}-L_{0}$: error in angular momentum over time $t$, and (\Romannum{3}) $A_{t}-A_{0}$: error in norm of the Laplace–Runge–Lenz vector function over time $t$.}
    	\label{fig:Kepler_Evolution_conserved_quantities}
    \end{figure}
     
    \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_SSPRKs3p3_ErrorVsTime_dt5e-03_tf200.eps}
         \caption{Third order method of Shu \& Osher, $\Delta t = 0.005$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_Fehlbergs6p4_ErrorVsTime_dt5e-02_tf200.eps}
         \caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/KEP/Kepler_DP5s7p5_ErrorVsTime_dt1e-01_tf200.eps}
          \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth in time by different methods for Kepler's Two-Body problem.}
    	\label{fig:Kepler_error_growth}
    \end{figure}
    Together with the baseline methods, the relaxation versions of these methods now require two more "independent" embedded methods to solve the system as it has three conserved quantities. The new embedded methods are provided in the appendix ~\ref{app:butcherTableau}, each having one less order of accuracy than the corresponding baseline method. Figure ~\ref{fig:Kepler_Evolution_conserved_quantities} demonstrates the advantage of relaxation over baseline RK methods. All the relaxation methods conserve three quantities almost to machine precision, while the baseline RK methods conserve them to around four decimal places. The consequence of these results is reflected in the asymptotic error growth by these methods, shown in Figure ~\ref{fig:Kepler_error_growth}. It shows a quadratic error growth by the baseline methods, while the corresponding invariants preserving (specifically the Hamiltonian) relaxation RK methods achieve a linear error growth over a long time.
    
    \subsubsection{Perturbed Kepler's Problem}
    The governing equations of the perturbed Kepler's problem are given by the following system
    \begin{subequations}\label{Eq:Perturbed_Kepler_problem}
        \begin{align}
            \dot{q_{1}} & = p_{1} \\
            \dot{q_{2}} & = p_{2} \\
            \dot{p_{1}} & = -\frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}} -\mu \frac{q_{1}}{\left(q_{1}^2+q_{2}^2\right)^{5/2}} \\
            \dot{p_{2}} & =-\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{3/2}}  -\mu\frac{q_{2}}{\left(q_{1}^2+q_{2}^2\right)^{5/2}} \;,
        \end{align}
    \end{subequations}
    where $\mu$ is a small number taken as $0.005$ for our numerical studies. Previous studies of this problem show that it is important for a numerical method to preserve both the invariants
    \begin{subequations} \label{Eq:Perturbed_Kepler_invariants}
        \begin{align}
            H(q,p) & = \frac{1}{2}\left(p_{1}^2+p_{2}^2\right)-\frac{1}{\sqrt{q_{1}^2+q_{2}^2}}-\frac{\mu}{2\sqrt{\left(q_{1}^2+q_{2}^2\right)^3}}\ (\text{Hamiltonian}) \\
        	L(q,p) & = q_{1}p_{2}-q_{2}p_{1}\ (\text{angular momentum}) \;,
        \end{align}
    \end{subequations}
    to capture the correct behavior of the solution. With the same initial conditions as in Kepler's two-body problem above but with a different eccentricity $e=0.6$, we solve the system using the baseline and the relaxation versions of the third order method of Shu \& Osher with $\Delta t = 0.03$, fourth order method of Fehlberg with $\Delta t = 0.05$, and fifth order method of Prince \& Dormand with $\Delta t = 0.1$. An expression of the analytical solution for the perturbed Kepler problem is not available, so we compute a proxy of the true solution by the dense output of the Python ”dopri5” method with minimal values for the relative and absolute tolerances. This gives us highly accurate solutions that allow us to study the long-time error growth behavior by different RK methods and their relaxation versions. The errors in both invariants and the numerical solutions of the orbits are presented in Figure ~\ref{fig:Perturbed_Kepler_Evolution_conserved_quantities} and Figure ~\ref{fig:Per_Kepler_error_growth}, respectively.

  \begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_SSPRKs3p3_InvariantVsTime_dt5e-02_tf300.eps}
        \caption{Third order method of Shu \& Osher, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Fehlbergs6p4_InvariantVsTime_dt5e-02_tf300.eps}
        \caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_DP5s7p5_InvariantVsTime_dt1e-01_tf300.eps}
        \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
        \caption{Errors in conserved quantities \eqref{Eq:Perturbed_Kepler_invariants} by different methods for perturbed Kepler's problem. (\Romannum{1}) $H_{t}-H_{0}$: error in Hamiltonian over time $t$, (\Romannum{2}) $L_{t}-L_{0}$: error in angular momentum over time $t$.}
        \label{fig:Perturbed_Kepler_Evolution_conserved_quantities}
    \end{figure}
    
    \begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_SSPRKs3p3_Sol_dt5e-02_tf300.eps}
        %\caption{Third order method of Shu \& Osher, $\Delta t = 0.03$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_Fehlbergs6p4_Sol_dt5e-02_tf300.eps}
        %\caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Baseline_DP5s7p5_Sol_dt1e-01_tf300.eps}
        %\caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_SSPRKs3p3_Sol_dt5e-02_tf300.eps}
        %\caption{Third order method of Shu \& Osher, $\Delta t = 0.03$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_Fehlbergs6p4_Sol_dt5e-02_tf300.eps}
        %\caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Relaxation_DP5s7p5_Sol_dt1e-01_tf300.eps}
        %\caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_SSPRKs3p3_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Fehlbergs6p4_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_DP5s7p5_LastFewStepsSolComp_tf300.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kepler_Exact_Orbit_dt3e-02_tf300.eps}
    \end{subfigure}
    	\caption{Solution of perturbed Kepler's problem by different methods. The first three plots in the last row of the figure compare the body's position by different methods at the few last steps of the simulation.}
    	\label{fig:Perturbed_Kepler_Solutions}
    \end{figure}
     Figure ~\ref{fig:Perturbed_Kepler_Evolution_conserved_quantities} shows that all the relaxation methods preserve the invariants up to the machine's precision as opposed to the underlying baseline methods and correctly produce the elliptic orbit that precesses slowly around one of its foci (Figure ~\ref{fig:Perturbed_Kepler_Solutions}). Note that the effect of preserving the conserved quantities by relaxation approach is only noticeable for the third-order method, where the baseline third-order method incorrectly captures the motion of orbits. Even though visually, the higher-order methods appear to produce the correct behavior of the trajectories without relaxation, in truth, these methods give completely wrong positions as time grows. As can be seen in Figure ~\ref{fig:Per_Kepler_error_growth}, the error of the baseline method increases quadratically with time until it reaches a saturation point of $100$\% error, leading to incorrect orbits of the body. The invariant-preserving relaxation approach, in contrast, results in a linear accumulation of error over time, which leads to a significantly smaller error, producing correct orbits of the body for a long time. 
     
     \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_SSPRKs3p3_ErrorVsTime_dt5e-02_tf300.eps}
         \caption{Third order method of Shu \& Osher, $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_Fehlbergs6p4_ErrorVsTime_dt5e-02_tf300.eps}
         \caption{Fourth order method of Fehlberg, $\Delta t = 0.05$.}
         %\label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/PER_KEP/Per_Kep_DP5s7p5_ErrorVsTime_dt1e-01_tf300.eps}
          \caption{Fifth order method of Prince \& Dormand, $\Delta t = 0.1$.}
         %\label{fig:}
     \end{subfigure}
    	\caption{Error growth in time by different methods for perturbed Kepler's Two-Body problem.}
    	\label{fig:Per_Kepler_error_growth}
    \end{figure}
    
   %\subsubsection{The Outer Solar System}
    % As an N-body system, we consider the outer-solar system that describes the motion of the outer planets (The Sun, Jupiter, Saturn, Uranus, Neptune, and Pluto) via the Hamiltonian
    % \begin{align}
    %     H(p, q)=\frac{1}{2} \sum_{i=0}^{5} \frac{1}{m_{i}} p_{i}^{T} p_{i}-G \sum_{i=1}^{5} \sum_{j=0}^{i-1} \frac{m_{i} m_{j}}{\left\|q_{i}-q_{j}\right\|} \;,
    % \end{align}
    % where $m_i$'s are the masses of the planets and the Sun, $p$ and $q$ are the supervectors consisting of the momenta and position vectors $p_{i},q_{i} \in \Real^{3}$, respectively. This system also admits the conservation of the angular momentum $L(p,q) = \sum_{i=0}^{5} q_{i} \times p_{i}$, which consists of three first integrals $L_{x},L_{y}$, and $L_{z}$:
    % \begin{align}
    %     L(p,q) = \sum_{i=0}^{5} q_{i} \times p_{i} 
    %     = \begin{bmatrix}
    %       L_{x} \\
    %       L_{y} \\
    %       L_{z}
    %      \end{bmatrix}
    %      = \begin{bmatrix}
    %       \sum_{i=0}^{5}\left(p_{i3} q_{i2}-p_{i2} q_{i3}\right) \\
    %       \sum_{i=0}^{5}\left(p_{i1} q_{i3}-p_{i3} q_{i1}\right) \\
    %       \sum_{i=0}^{5}\left(p_{i2} q_{i1}-p_{i1} q_{i2}\right)
    %      \end{bmatrix} \;,
    % \end{align}
    % where $p_{ij},q_{ij} $ are the $j$-th component of momenta and position of the $i$-th planet. We conduct numerical studies with the parameters of the problem and the initial conditions given as in \cite[Section I.2.3]{haier2006geometric}. 
    %   \begin{figure}[ht]
    %  \centering
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{img/outer_Solar_Heuns3p3_InvariantVsTime_dt200_tf200000.eps}
    %      \caption{Third order method of Heun, $\Delta t = 400$.}
    %      %\label{fig:}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{img/outer_Solar_Fehlbergs6p4_InvariantVsTime_dt400_tf200000.eps}
    %      \caption{Fourth order method of Fehlberg, $\Delta t = 500$.}
    %      %\label{fig:}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{img/outer_Solar_DP5s7p5_InvariantVsTime_dt400_tf200000.eps}
    %      \caption{Fifth order method of Prince \& Dormand, $\Delta t = 500$.}
    %      %\label{fig:}
    %  \end{subfigure}
    % 	\caption{Errors in the Hamiltonian and the angular moemntum by different methods for the outer solar system. (\Romannum{1}) $H_{t}-H_{0}$: error in Hamiltonian over time $t$, (\Romannum{2}) $L_{t}-L_{0}$: error in angular momentum over time $t$.}
    % 	\label{fig:Outer_Solar_Evolution_conserved_quantities}
    % \end{figure}

    \subsection{Korteweg–De Vries (KdV) equation}
     As an example of a PDE problem, we consider the Kortweg-de Vries equation on a periodic domain in $1$D  
    \begin{align}\label{KdV_Equation}
        u_t+6uu_x+u_{xxx} & = 0, \ \text{on} \ [x_{L},x_{R}]\times(0,T] \;, \\
    \end{align}
    which has soliton solutions and infinitely many conserved quantities, making it a very good test problem for our numerical methods. Mass and energy are the two important conserved quantities of the kdV equation that are mostly considered for numerical studies in the literature. For the 1-soliton solution of the KdV equation, the mass and energy preserving methods are proved to have linearly growing error behavior. In contrast, the nonconservative schemes produce errors that grow quadratically \cite{de1997accuracy}. For the 2-soliton case, a similar error growth behavior is observed by mass and energy-conserving methods vs. nonconservative methods. It is well-known that linear invariants are preserved by all the RK methods. To demonstrate that the relaxation methods can preserve multiple invariants for PDE problems, which is also necessary for better error growth over time in some multi-soliton solutions, together with the mass and energy, we consider another nonlinear invariant discovered by Whitham \cite{strang1986introduction}, given in equation \eqref{KdV_invariants}.
    \begin{subequations} \label{KdV_invariants}
        \begin{align}
            \int u \ dx \ (\text{mass}) \\
        	\int \frac{1}{2} u^2 \ dx \ (\text{energy}) \\
        	\int \left(2u^3 -u_x^2  \right) dx \ (\text{Whitham}) \;.
        \end{align}
    \end{subequations}
    We consider different spatial semidiscretizations of the KdV equation for n-soliton with $n = 1,2,3$ that conserve different combinations of invariants from \eqref{KdV_invariants} and study the error propagation mechanism by time integrators along with their relaxation versions. The third derivative in space in the KdV equation makes the semi-discretization a stiff ODE system, so we choose ImEx time integrators as the baseline methods and compare the numerical results with their relaxation versions. For all the case studies of the KdV equation, two ImEx methods, a third-order ImEx method with a second-order embedded pair  and a fourth-order ImEx method with a third-order embedded pair \cite[Appendix C]{kennedy2003additive}, are used with different time steps (see figures) to compute the numerical solutions.
    
    \subsubsection{Relaxation Methods on Conservative Semi-discretized KdV System}
    First, we take a mass and energy preserving spatial approximation given in \cite{ranocha2020relaxation} on the periodic domain $[x_{L},x_{R}]$ using the pseudo-spectral method and a split form based on SBP operators \cite{ranocha2006broad}
    \begin{equation}\label{SBP_semi_discretization}
       \partial_{t} U+6 \times \frac{1}{3}\left(D_{1}(U \cdot U)+U \cdot\left(D_{1} U\right)\right)+D_{3} U=0,
    \end{equation}
    where $D_k$ approximates the $k$th derivative of the grid function $U$ on the spatial grid points and $\cdot$ here acts as elementwise multiplication. The solution to this discretized system \ref{SBP_semi_discretization} satisfies the discrete analogous of \ref{KdV_invariants} for mass and energy \cite{ranocha2020relaxation} as 
    \begin{subequations} \label{KdV_discrete_inv_mass_energy}
        \begin{align}
            \frac{\mathrm{d}}{\mathrm{dt}}\left[dx \sum_{j}U_j\right] = 0 \\
            \frac{\mathrm{d}}{\mathrm{dt}}\left[dx \sum_{j}|U_j|^2\right] = 0 \;.
        \end{align}
    \end{subequations}
    With this semi-discretization \ref{SBP_semi_discretization}, we apply the relaxation approach to the KdV equation with different soliton solutions (see appendix \ref{app:soliton-solutions}) to demonstrate the conservation of the invariants (mass and energy) and the error growth behavior over time. Since mass is a linear invariant, it is conserved by RK methods, so we only impose invariant conditions on nonlinear invariants in the relaxation RK approach.
    
    Let us now consider the 1-soliton solution ((a) in appendix \ref{app:soliton-solutions}) on the domain $[x_{L},x_{R}]=[-20,60]$ of length $L = 80$. We use the above semi-discretization with $N=512$ spatial grid points and integrate from $t=0$ to $t=20$. Table ~\ref{Table:1_invariant_error} displays the values of maximum errors in different invariants, and it clearly shows all the relaxation RK methods preserve both the invariants for different n-soliton solutions. In Figure ~\ref{fig:KdV_1_sol_1_inv_GlobalErrors}, we plot the global error as a function of time. The errors behave linearly for RK methods with relaxation and quadratically without relaxation. These numerical results agree with the analytical results presented in \cite{de1997accuracy}, i.e., in the case of 1-soliton solution of the KdV equation, the errors incurred by methods conserving mass and energy grow linearly as opposed to quadratic growth by non-conservative methods.
    \begin{table}
    \centering
    \begin{tabular}{ | c | c | c | c | c |}
        \hline
               &    &          \multicolumn{3}{c}{Invariant Error in}\\
        \hline
        Case & Methods & Mass & Energy & Whitham  \\
        \hline
        \multirow{4}*{1-soliton and 1 invariant} & Baseline ImEx (3,2)  & $1.18e-13$ & $5.38e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $1.19e-13$ & $2.22e-16$ &  \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $1.04e-13$ & $1.05e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $1.06e-13$ & $3.33e-16$ &  \\
        \hline
        \multirow{4}*{2-soliton with 1 invariant} & Baseline ImEx (3,2)  & $9.50e-14$ & $1.10e-01$ & \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $8.97e-14$ & $4.44e-16$ & \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $5.68e-14$ & $2.32e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $5.86e-14$ & $8.88e-16$ &  \\
        \hline 
        % \multirow{4}*{2-soliton with 2 invariants} & Baseline ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Baseline ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \hline 
        \multirow{4}*{3-soliton with 1 invariant} & Baseline ImEx (3,2)  & $6.57e-14$ & $2.07e-01$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (3,2)  & $7.19e-14$ & $2.22e-16$ &  \\
        \cline{2-5}
                             & Baseline ImEx (4,3)  & $3.82e-14$ & $4.62e-02$ &  \\
        \cline{2-5}
                             & Relaxation ImEx (4,3)  & $3.73e-14$ & $8.88e-16$ &  \\
        \hline
        % \multirow{4}*{3-soliton with 2 invariants} & Baseline ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (3,2)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Baseline ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \cline{2-5}
        %                      & Relaxation ImEx (4,3)  & $1$ & $2$ & $4$ \\
        % \hline 
    \end{tabular}
    \caption{Maximum invariant errors by various methods for different n-solitons with 1 invariant case.}
    \label{Table:1_invariant_error}
    \end{table}
     
    %  \begin{table} \small%
    %     \begin{tabular}{| c | c | c | c | c |}
    %     \hline
    %     Case & Methods & Mass & Energy & Whitham  \\
    %     \hline
    %     \cline{2-4}
    %                      & Second solution & Data 1 & Yes \\
    %                      &                & Data 2 &  \\
    %                      &                & Data 3 &  \\
    %     \hline
    %     \end{tabular}
    % \end{table}
    
    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_1_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf20.eps}
        \caption{Third order additive Runge-Kutta (ARK) method with  second order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_1_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf20.eps}
        \caption{Fourth order ARK method with third order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Error growth against time by different method for the KdV equation  with 1-soliton solution and 1 invariant case. Red dotted line: baseline ARK method, i.e., ARK method without relaxation and solid green line: ARK method with relaxation.}
	\label{fig:KdV_1_sol_1_inv_GlobalErrors}
    \end{figure}
    Next, we consider a 2-soliton solution over the region $[x_{L},x_{R}]=[-80,80]$ and use the semi-discretization \eqref{SBP_semi_discretization} with $N=768$ spatial grid points. The resulting system is solved by different time integrators starting from $t=-25$ to $t=25$. The error growth behavior by the numerical methods is presented in Figure ~\ref{fig:KdV_2_sol_1_inv_GlobalErrors}. \abhi{How do we explain such error growth behavior for the 2-soliton 1-invariant case?} Similar numerical experiments are carried out in the case of a 3-soliton solution on the domain $[x_{L},x_{R}]=[-130,130]$ with $N=1024$ spatial grid points. We integrate the discretized system by two ARK methods from $t=-50$ to $t=50$. Figure ~\ref{fig:KdV_3_sol_1_inv_GlobalErrors} shows the errors over time by different ARK methods. Unlike the 1-soliton solution case, here, the conservative relaxation approach results in quadratic growth of errors similar to baseline ARK methods. This indicates that the mass and the energy preserving relaxation methods produce only a better error for a 3-soliton solution but fail to improve the asymptotic error growth compared to the baseline methods. We observed linearly decreasing amplitude errors and hence quadratically growing phase errors for all three solitons of different amplitudes, which is responsible for the overall quadratic error growth for the 3-soliton solutions.
     
    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf25.eps}
        \caption{Third order ARK method with a second order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf25.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Error growth against time by different method for the KdV equation  with 2-soliton solution and 1 invariant case. Red dotted line: baseline ARK method, i.e., ARK method without relaxation and solid green line: ARK method with relaxation.}
	\label{fig:KdV_2_sol_1_inv_GlobalErrors}
    \end{figure}
    
    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_1_inv_ARK32_ErrorVsTime_dt1e-01_tf50.eps}
        \caption{Third order ARK method with a second order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_1_inv_ARK43_ErrorVsTime_dt1e-01_tf50.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.1$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Error growth against time by different method for the KdV equation  with 3-soliton solution and 1 invariant case. Red dotted line: baseline ARK method, i.e., ARK method without relaxation and solid green line: ARK method with relaxation.}
	\label{fig:KdV_3_sol_1_inv_GlobalErrors}
    \end{figure}
    %  where the amplitudes are $A_1=2$, $A_2=1$, and $A_3=0.5$.
    %  For all the case studies of the KdV equation, two ImEx methods, a third-order ImEx method \abhi{reference} with a second-order embedded pair (see Appendix) and a fourth-order ImEx method \abhi{reference} with a third-order embedded pair (see Appendix), are used with different time steps (see figures) to compute the numerical solutions with and without relaxation. The composite Simpson rule is used to calculate the values of invariants at each step to accurately capture the errors in conserved quantities, which is crucial, especially for the relaxation approach. The reference solution is computed by using the dense output of the Python "dopri5" method with minimal values for the relative and absolute tolerances and then compared with numerical solutions by different methods. 
    %  \abhi{Add numerical results for 2 and 3 solitons here.}
    %  In figures 1 and 2 we display the change in invariants by different methods for 2 and 3 soliton, respectively. In both cases relaxation approach preserve the invariants under consideration. The error propagations are presented in figures 3 and 4. In line with \cite{de1997accuracy}, figure 3 shows a linear growth of error before and after interaction for the 2-soliton case  by conservative relaxation method. For the nonconservative ImEx method, the error growth is quandratic. Similar error propagation mechanism is observed for the 3-soliton case in figure 4.
     \subsubsection{Relaxation Methods on Non-conservative Semi-discretized KdV System}
    As we have seen that conserving only two invariant quantities (mass and energy) is not enough to produce linear error growth for the 2 and 3-soliton solutions, we now focus on the third nonlinear invariant. Since we do not have a semi-discretization that preserves the energy and the Whitham's invariant, we employ the same pseudospectral spatial discretization as in \eqref{SBP_semi_discretization}. With this semi-discretized system, we compute the Whitham's invariant using the composite Simpson rule, in which the first derivative is calculated using the discrete Fourier transform. The composite Simpson rule is used to calculate the values of Whitham's invariant to accurately capture the errors in this conserved quantity, which is crucial, especially for the relaxation approach. We choose the number of spatial grid points so that no further error reduction can be obtained in the time derivative of Whitham's invariant by taking more grid points. This requires $N = 1024$ grid points for a 2-soliton solution on the domain $[-80,80]$ and $N = 1536$ grid points for a 3-soliton solution on the domain $[-130,130]$. %This allows us to study the error behavior solely by the time-stepping methods.
    Even though we do not have a conservative semi-discretized system, our goal here is to study the performance of the relaxation approach on a non-conservative system via this example. Like all the examples above, we also use the python 'fsolve' to find the solution for the relaxation parameters at each step of our numerical method. We observe that the 'fsolve' method fails to find a solution to the invariant equations at many steps in our numerical simulation. In these cases, we further use the Python 'brute' method to find a good initial guess for the Python 'fmin' method and find a solution for relaxation parameters that minimizes the sum of squares of the invariant equations. Finally, we choose the solution with a better residual error among the two solutions given by the two methods.

    Figures ~\ref{fig:KdV_2_sol_2_inv_InvariantErrors} and ~\ref{fig:KdV_3_sol_2_inv_InvariantErrors} show the error in invariants over time for multi-soliton solutions by different ARK methods. Relaxation methods improve the error in invariants, but they are not up to the machine accuracy. The error growth behavior for multi-soliton solutions in Figures ~\ref{fig:KdV_2_sol_2_inv_GlobalErrors} and ~\ref{fig:KdV_3_sol_2_inv_GlobalErrors} demonstrates the advantage of relaxation methods over baseline methods for a long time numerical solution.
    
    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK32_ErrorVsTime_dt1e-02_tf25.eps}
        \caption{Third order ARK method with a second order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK43_ErrorVsTime_dt1e-02_tf25.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Error growth against time by different method for the KdV equation  with 2-soliton solution and 2 invariant case. Red dotted line: baseline ARK method, i.e., ARK method without relaxation and solid green line: ARK method with relaxation.}
	\label{fig:KdV_2_sol_2_inv_GlobalErrors}
    \end{figure}

    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK32_ErrorVsTime_dt1e-02_tf50.eps}
        \caption{Third order ARK method with a second order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK43_ErrorVsTime_dt1e-02_tf50.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Error growth against time by different method for the KdV equation  with 3-soliton solution and 2 invariant case. Red dotted line: baseline ARK method, i.e., ARK method without relaxation and solid green line: ARK method with relaxation.}
	\label{fig:KdV_3_sol_2_inv_GlobalErrors}
    \end{figure}

    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK32_InvariantVsTime_dt1e-02_tf25.eps}
        \caption{Third order ARK method with a second order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_2_sol_2_inv_dt1e-02_ARK43_InvariantVsTime_dt1e-02_tf25.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Errors in invariants by different method for the KdV equation  with 2-soliton solution and 2 invariant case. (\Romannum{1}) $\eta_{0}(t)-\eta_{0}(0)$: error in mass over time $t$, (\Romannum{2}) $\eta_{1}(t)-\eta_{1}(0)$: error in energy over time $t$, and (\Romannum{3}) $\eta_{0}(t)-\eta_{0}(0)$: error in the Whitham's invariant over time $t$.}
	\label{fig:KdV_2_sol_2_inv_InvariantErrors}
    \end{figure}

    \begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK32_InvariantVsTime_dt1e-02_tf50.eps}
        \caption{Third order ImEx method second order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/KdV/KdV_3_sol_2_inv_dt1e-02_ARK43_InvariantVsTime_dt1e-02_tf50.eps}
        \caption{Fourth order ARK method with a third order embedding, $\Delta t = 0.01$.}
        %\label{fig:}
    \end{subfigure}
	\caption{Errors in invariants by different method for the KdV equation with 3-soliton solution and 2 invariant case. (\Romannum{1}) $\eta_{0}(t)-\eta_{0}(0)$: error in mass over time $t$, (\Romannum{2}) $\eta_{1}(t)-\eta_{1}(0)$: error in energy over time $t$, and (\Romannum{3}) $\eta_{0}(t)-\eta_{0}(0)$: error in the Whitham's invariant over time $t$.}
	\label{fig:KdV_3_sol_2_inv_InvariantErrors}
    \end{figure}


    
%     \section{KdV Numerical Results}
%     Numerical results out of different experiments on KdV equation:
%     \subsection{KdV with 1-soliton 1 invariant}
%     This is ...
%     \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_1_inv_ImEx32_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_1_inv_ImEx43_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_1_inv_ImEx32_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_1_inv_ImEx43_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 1-soliton solution and $1$ invariant case (top). Error growth against time by different method for the KdV equation  with 1-soliton solution and $1$ invariant case (bottom).}
% 	\label{fig:KdV_1_sol_1_inv_InvariantErrors_GlobalErrors}
%     \end{figure}
    
%     \subsection{KdV with 2-soliton 1 invariant}
%     This is ...
%     \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_2_sol_1_inv_ImEx32_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_2_sol_1_inv_ImEx43_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_2_sol_1_inv_ImEx32_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_2_sol_1_inv_ImEx43_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 2-soliton solution and $1$ invariant case (top). Error growth against time by different method for the KdV equation  with 2-soliton solution and $1$ invariant case (bottom).}
% 	\label{fig:KdV_2_sol_1_inv_InvariantErrors_GlobalErrors}
%     \end{figure}

%   \subsection{KdV with 3-soliton 1 invariant}
%     This is ...
%     \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx32_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx43_InvariantVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx32_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx43_ErrorVsTime_dt1e-01_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 3-soliton solution and $1$ invariant case (top). Error growth against time by different method for the KdV equation  with 3-soliton solution and $1$ invariant case (bottom).}
% 	\label{fig:KdV_3_sol_1_inv_InvariantErrors_GlobalErrors_case_1}
%     \end{figure}
%     \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx32_InvariantVsTime_dt2e-02_tf400.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.02$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx43_InvariantVsTime_dt5e-02_tf400.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.05$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx32_ErrorVsTime_dt2e-02_tf400.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.02$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_3_sol_1_inv_ImEx43_ErrorVsTime_dt5e-02_tf400.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.05$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 3-soliton solution and $1$ invariant case (top). Error growth against time by different method for the KdV equation  with 3-soliton solution and $1$ invariant case (bottom).}
% 	\label{fig:KdV_3_sol_1_inv_InvariantErrors_GlobalErrors_case_2}
%     \end{figure}
    
%     \subsection{KdV with 1-soliton 2 invariants}
%     This is ...
%     \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_2_inv_ImEx32_InvariantVsTime_dt1e-02_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.01$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_2_inv_ImEx43_InvariantVsTime_dt2e-02_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.02$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_2_inv_ImEx32_ErrorVsTime_dt1e-02_tf1000.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.01$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/KdV_1_sol_2_inv_ImEx43_ErrorVsTime_dt2e-02_tf1000.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.02$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 1-soliton solution and $2$ invariants case (top). Error growth against time by different method for the KdV equation  with 1-soliton solution and $2$ invariants case (bottom).}
% 	\label{fig:KdV_1_sol_2_inv_InvariantErrors_GlobalErrors}
%     \end{figure}

% \section{KdV Numerical Results}
%     Numerical results out of different experiments on KdV equation:
%     \subsection{KdV with 2-soliton 1 invariant}
%     \begin{align}
%         u_t+6uu_x+u_{xxx} & = 0, \ \text{on} \ [-60,60]\times(-10,20] \;, \\
%     \end{align}
%     The KdV 2-soliton solution is
%     \begin{align*}
%         u(x, t) = \frac{2\left(c_1-c_2\right)\left(c_1 \cosh ^2\left(\sqrt{ } c_2 \xi_2 / 2\right)+c_2 \sinh ^2\left(\sqrt{ } c_1 \xi_1 / 2\right)\right)}{\left(\sqrt{ } c_1-\sqrt{ } c_2\right) \cosh \left(\left(\sqrt{ } c_1 \xi_1+\sqrt{ } c_2 \xi_2\right) / 2\right)} + \\ 
%         \left(\sqrt{ } c_1+\sqrt{ } c_2\right) \cosh \left(\left(\sqrt{ } c_1 \xi_1-\sqrt{ } c_2 \xi_2\right) / 2\right)^2 \;.
%     \end{align*}
%     where $c_1>c_2>0$ are the wave speeds and $\xi_1=x-c_1 t, \xi_2=x-c_2 t$ are moving coordinates. $c_1=2,c_2=1$.
%     \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{KdV2img/KdV_2_sol_1_inv_ImEx32_InvariantVsTime_dt1e-01_tf20.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{KdV2img/KdV_2_sol_1_inv_ImEx43_InvariantVsTime_dt1e-01_tf20.eps}
    %     \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{KdV2img/KdV_2_sol_1_inv_ImEx32_ErrorVsTime_dt1e-01_tf20.eps}
%         \caption{Third order ImEx method second order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{KdV2img/KdV_2_sol_1_inv_ImEx43_ErrorVsTime_dt1e-01_tf20.eps}
%         \caption{Fourth order ImEx method third order embedding, $\Delta t = 0.1$.}
%         %\label{fig:}
%     \end{subfigure}
% 	\caption{Errors in invariants by different method for the KdV equation with 2-soliton solution and $1$ invariant case (top). Error growth against time by different method for the KdV equation  with 2-soliton solution and $1$ invariant case (bottom).}
% 	\label{fig:KdV_1_sol_1_inv_InvariantErrors_GlobalErrors}
%     \end{figure}

    
\section{Conclusions}
In this work, we propose a generalization of the relaxation framework for RK methods to preserve multiple nonlinear conserved quantities of a dynamical system. We prove the existence of the relaxation parameters and the accuracy of the generalized relaxation methods under some conditions. Depending on the system's stiffness, the generalized relaxation approach is applied with different RK methods, such as explicit RK and additive RK methods. Numerical results demonstrate that the generalized relaxation RK methods can conserve multiple conserved quantities and produce qualitatively better numerical solutions. 

An important case study of our numerical experiments includes the KdV equation with multi-soliton solutions. With a conservative semi-discretization of the KdV equation preserving mass and energy, the relaxation approach applied with ARK methods successfully preserves the invariants for 1, 2, and 3-soliton solutions. We observe that mass and energy preservation do not produce linear error growth for multi-soliton solutions for the KdV equation. Some numerical results applying relaxation methods to a non-conservative semi-discretization (enforcing conservation of a third nonlinear invariant ) of the KdV equation are presented. Numerical results suggest that relaxation methods can be advantageous if we are interested in long time numerical solutions. 

The application of this general relaxation framework to the nonlinear Schr\"{o}dinger equation with multiple nonlinear invariants is a subject of ongoing research. Another possible research direction is extending the generalized relaxation approach framework to the other class of time integration schemes, such as linear multistep methods, and improving the underlying methods' numerical performance.
%================================================================================
\appendix
%================================================================================
\section{List of RK Methods} 
\label{app:butcherTableau}
%================================================================================

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{3cm}{!}{%
    	\begin{tabular}{l|l l}
             0  &    0 \\                        
             1  &    1  &   0  \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/2  &   1/2 \\
             \hline
            $\vec{b}^{\,2}$  &   1/3  &   2/3	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{SSPRK(2,2): Second-order method $(A,\vec{b}^{\,1})$ with first-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_ssprk22}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{10cm}{!}{%
    	\begin{tabular}{l|l l l}
             0  &    0 \\                        
             1  &    1  &   0  \\ 
             1/2 &          1/4   &        1/4 & 0 \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/6  &          1/6    &        2/3   \\
             \hline
            $\vec{b}^{\,2}$  &   0.246284400816981 &   0.246284400816981  &  0.507431198366038	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{SSPRK(3,3): Third-order method $(A,\vec{b}^{\,1})$ with second-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_ssprk33}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{10cm}{!}{%
    	\begin{tabular}{l|l l l}
             0  &    0 \\                        
             1/3  &    1/3  &   0  \\ 
             2/3 &      0   &    2/3 & 0 \\ 
             \hline
            $\vec{b}^{\,1}$  &   1/4  &          0   &        1/4   \\
             \hline
            $\vec{b}^{\,2}$  &   0.006419303047187  & 0.487161393905626 &  0.506419303047187	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{Heun(3,3): Third-order method $(A,\vec{b}^{\,1})$ with second-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_heun33}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{5cm}{!}{%
    	\begin{tabular}{l|l l l l}
             0  &    0 \\                        
             1/2  &    1/2  &   0  \\ 
             1/2 &      0   &    1/2 & 0 \\ 
             1   &      0   &    0   &     1      &    0  \\
             \hline
            $\vec{b}^{\,1}$  &   1/6   &        1/3    &       1/3      &     1/6  \\
             \hline
            $\vec{b}^{\,2}$  &   1/4   &        1/4      &     1/4     &      1/4	 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{RK(4,4): Fourth-order method $(A,\vec{b}^{\,1})$ with second-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_rk44}
\end{table}

% \begin{table}[H]
%     \centering
%     \begin{adjustbox}{angle=0}
%     \resizebox{10cm}{!}{%
%     	\begin{tabular}{l|l l l l l l l l l l}
%              0    &    0 \\                        
%              1/6  &          1/6   &          0  \\ 
%              1/3  &          1/6   &         1/6   &          0 \\
%              1/2  &          1/6   &         1/6   &         1/6   &          0 \\ 
%              2/3  &          1/6   &        1/6    &        1/6    &        1/6   &     0 \\
%              1/3  &          1/15  &         1/15  &         1/15  &         1/15  &         1/15 &           0\\
%              1/2  &          1/15  &        1/15   &        1/15   &        1/15   &        1/15      &     1/6   &          0 \\
%              2/3  &          1/15  &          1/15  &         1/15  &         1/15  &         1/15  &         1/6  &          1/6    &         0 \\
%              5/6   &         1/15  &         1/15  &         1/15   &        1/15   &        1/15   &        1/6    &        1/6    &        1/6     &        0 \\
%               1     &        1/15   &        1/15   &        1/15    &       1/15   &       1/15      &     1/6      &      1/6    &        1/6    &        1/6  &           0\\
             
%              \hline
%             $\vec{b}^{\,1}$  &   1/10     &      1/10   &        1/10   &        1/10  &         1/10   &        1/10    &       1/10    &       1/10    &       1/10     &      1/10  \\
%              \hline
%             $\vec{b}^{\,2}$ & 0    &         2/9   &          0     &         0    &         5/18   &       1/3    &         0   &           0      &        0      &       1/6     			  	 
%     	\end{tabular}%
%     	}%
%     \end{adjustbox}
%     \caption{SSPRK(10,4): Fourth-order method $(A,\vec{b}^{\,1})$ with third-order embedded method $(A,\vec{b}^{\,2})$.}
%     \label{tab:BT_ssprk104}
% \end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{18cm}{!}{%
    	\begin{tabular}{l|l l l l l l}
             0  &    0 \\                        
             1/4 &          1/4  &          0   \\ 
             3/8 &	3/32 &	9/32 & 0 \\ 
             12/13	& 1932/2197 & 	-7200/2197 &	7296/2197 &   0\\
             	1 &	439/216 &	-8 &	3680/513 &	-845/4104 &    0\\
              1/2 &	-8/27  &	2 &	-3544/2565 &	1859/4104 &	-11/40 &	    0\\
             \hline
            $\vec{b}^{\,1}$  &  25/216 &	0 &	1408/2565 &	2197/4104  &	-1/5  &	0   \\
             \hline
            $\vec{b}^{\,2}$  &   0.122702088570621 &   0.000000000000003 &  0.251243531398616 & -0.072328563385151 &  0.246714063515406 &  0.451668879900505 				   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{Fehlberg(5,4): Fourth-order method $(A,\vec{b}^{\,1})$ with third-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_fehlberg54}
\end{table}

\begin{table}[H]
    \centering
    \begin{adjustbox}{angle=0}
    \resizebox{15cm}{!}{%
    	\begin{tabular}{l|l l l l l l l}
             0  &    0 \\                        
             1/5 &          1/5  &          0   \\ 
            3/10 & 	3/40 & 	9/40 & 0 \\ 
             4/5 & 	44/45 & 	-56/15 & 	32/9 &   0\\
            8/9	&  19372/6561 & 	-25360/2187 & 	64448/6561 & 	-212/729 &    0\\
            1	& 9017/3168  & 	-355/33	 &  46732/5247 & 	49/176 & 	-5103/18656 &	    0\\
            1	&  35/384  & 	0  & 	500/1113  & 	125/192 & 	-2187/6784 & 	11/84  &    0\\
             \hline
            $\vec{b}^{\,1}$  &  35/384 & 	0  & 	500/1113  & 	125/192  & 	-2187/6784  & 	11/84  & 	0   \\
             \hline
            $\vec{b}^{\,2}$  &   5179/57600  & 	0  & 	7571/16695  & 	393/640  & 	-92097/339200  &  187/2100  & 1/40			   			 
    	\end{tabular}%
    	}%
    \end{adjustbox}
    \caption{DP(7,5): Fifth-order method $(A,\vec{b}^{\,1})$ with Fourth-order embedded method $(A,\vec{b}^{\,2})$.}
    \label{tab:BT_dp54}
\end{table}
%================================================================================
\section{Soliton Solutions} 
\label{app:soliton-solutions}
Diffrent soliton solutions \cite{ranocha2020relaxation} of the KdV equation \eqref{KdV_Equation} are given below: 
\begin{enumerate}
    \item [(a)] \textbf{1-soliton solution}:
    \begin{align}
        u(x,t)= \beta_1 \sech ^2(\xi_1) \;,
    \end{align}
    where $\beta_1 = 1$ and $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$.
    \item [(b)] \textbf{2-soliton solution}:
    \begin{align}
        u(x, t) = -\frac{2(\beta_1-\beta_2)\left(\beta_2 \csch^2(\xi_2)+\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)\right)^2} \;,
    \end{align}
    where $\beta_1 = 0.5$, $\beta_2 = 1$, $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$, and $\xi_2 = \frac{\sqrt{\beta_2}(x-2 \beta_2 t)}{\sqrt{2}}$.
    \item [(c)] \textbf{3-soliton solution}:
    \begin{align}
        u(x, t) = \beta_1\sech^2(\xi_1)- \frac{2(\beta_2-\beta_3)\left(\frac{2(\beta_3-\beta_1)\left(\beta_3 \csch^2(\xi_3)-\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_3} \tanh(\xi_3)-\sqrt{2 \beta_1} \tanh(\xi_1)\right)^2}-\frac{2(\beta_1-\beta_2)\left(\beta_2 \csch^2(\xi_2)+\beta_1 \sech ^2(\xi_1)\right)}{\left(\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)\right)^2} \right)}{\left(\frac{2(\beta_1-\beta_2)}{\sqrt{2 \beta_1} \tanh(\xi_1)-\sqrt{2 \beta_2} \coth(\xi_2)}-\frac{2(\beta_3-\beta_1)}{\sqrt{2 \beta_3} \tanh(\xi_3)-\sqrt{2 \beta_1} \coth(\xi_1)}\right)^2}\;,
    \end{align}
    where $\beta_1 = 0.4$, $\beta_2 = 0.7$, $\beta_3 = 1$, $\xi_1 = \frac{\sqrt{\beta_1}(x-2 \beta_1 t)}{\sqrt{2}}$, $\xi_2 = \frac{\sqrt{\beta_2}(x-2 \beta_2 t)}{\sqrt{2}}$, and $\xi_3 = \frac{\sqrt{\beta_3}(x-2 \beta_3 t)}{\sqrt{2}}$.
\end{enumerate}

%================================================================================
%================================================================================
\section*{Acknowledgments}
%================================================================================

%================================================================================




%================================================================================

